Enhancing Workflow Security in Multi-Cloud Environments through Monitoring and Adaptation upon Cloud Service and Network Security Violations

Cloud computing has emerged as a crucial solution for handling data- and compute-intensive workflows, offering scalability to address dynamic demands. However, ensuring the secure execution of workflows in the untrusted multi-cloud environment poses significant challenges, given the sensitive nature of the involved data and tasks. The lack of comprehensive approaches for detecting attacks during workflow execution, coupled with inadequate measures for reacting to security and privacy breaches has been identified in the literature. To close this gap, in this work, we propose an approach that focuses on monitoring cloud services and networks to detect security violations during workflow executions. Upon detection, our approach selects the optimal adaptation action to minimize the impact on the workflow. To mitigate the uncertain cost associated with such adaptations and their potential impact on other tasks in the workflow, we employ adaptive learning to determine the most suitable adaptation action. Our approach is evaluated based on the performance of the detection procedure and the impact of the selected adaptations on the workflows.

==> Algorithms/LearningAdaptationActions.tex <==
\begin{algorithm}
\caption{Learning Adaptation Actions}
\label{alg:LearningAdaptationActions}
\begin{algorithmic} [1]
\REQUIRE $\mathcal{DS}$: {Adaptation_LogFile} 
\ENSURE  $\mathcal{M}$: Trained Model Learning Adaptation Actions
\FORALL{$\mathcal{TaskType}$ in $\mathcal{DS}$}
\STATE $\mathcal{TaskType}{\text{train}}, \mathcal{TaskType}{\text{test}} \gets$ Split($\mathcal{TaskType}$) into training and testing sets
\STATE $\mathcal{M_{TaskType}} \gets$ TrainRandomForest($\mathcal{TaskType}{\text{train}}$) 
\STATE $Accuracy_{\mathcal{M_{TaskType}}} \gets$ TestRandomForest($\mathcal{M_{TaskType}}, \mathcal{TaskType}{\text{test}}$) 
\ENDFOR
\RETURN $\mathcal{M}, Accuracy_{\mathcal{M}}$ 
\end{algorithmic}
\end{algorithm}

==> Algorithms/Periodic_Trust_Update_Algorithm_for_Providers.tex <==
\begin{algorithm}
\caption{Periodic Trust Update Algorithm for Providers}
\begin{algorithmic} [1]
\REQUIRE $\tau$: time period for updating trust (in seconds)
\ENSURE $TRP$: updated trust repository of providers
\STATE $APM \leftarrow TrainModel(CLF+NTD)$
\WHILE{system is operational}
\STATE $start_time  \leftarrow$ current system time
\STATE $TRP_{new}  \leftarrow$ empty dictionary
\FOR {each tenant $T_i$}
\STATE $TRP_i  \leftarrow$ trust data collected from tenant $T_i$
\FOR {each provider $P_j$ in $TRP_i$}
\IF {$P_j$ is not in $TRP_{new}$}
\STATE $TRP_{new}[P_j]  \leftarrow TRP_i[P_j]$
\Else
\STATE $TRP_{new}[P_j]  \leftarrow$ weighted average of $TRP_{new}[P_j]$ and $TRP_i[P_j]$

\ENDIF
\ENDFOR
\ENDFOR
\STATE $TRP \gets TRP_{new}$
\STATE $end_time \gets$ current system time
\STATE $sleep_time \gets \tau - (end_time - start_time)$
\STATE sleep for $sleep_time$ second
\ENDWHILE
\end{algorithmic}
\end{algorithm}


==> Algorithms/TrainingActionSelection.tex <==
\begin{algorithm}
\caption{Action Selection Trainer Algorithm}
\label{alg:TrainingActionSelectionAlgorithm}
\begin{algorithmic} [1]
\REQUIRE $Updates$: Updates from the Adaptation Decision Engine, $\mathcal{P}$: Time period
\ENSURE  $\mathcal{M}_{ActionSelection}$: Trained Model for Selecting the proper Adaptation Action
\STATE $\mathcal{D} \gets$ GenerateInitialLogfile() 
\WHILE{system is operational}
\STATE $\mathcal{D} \gets$ $\mathcal{D}+Updates$
\STATE $\mathcal{D}{\text{train}}, \mathcal{D}{\text{test}} \gets$ Split($\mathcal{D}$) into training and testing sets
\STATE $\mathcal{M_D} \gets$ TrainRandomForest($\mathcal{D}{\text{train}}$) 
\STATE $Accuracy_{\mathcal{M_D}} \gets$ TestRandomForest($\mathcal{M_D}, \mathcal{D}{\text{test}}$) 
\RETURN $\mathcal{M}, Accuracy_{\mathcal{M}}$ 
\STATE \textbf{Wait}($\mathcal{P}$)
\ENDWHILE
\end{algorithmic}
\end{algorithm}

==> Algorithms/check.tex <==
\begin{algorithm}
\caption{Service Monitoring Algorithm}
\label{alg:Service Monitoring Algorithm}
\begin{algorithmic}[1]
\REQUIRE $\mathcal{N}$: Real-time Network Traffic Data, $\mathcal{M}$: Trained Model for Attack Detection, $severity$: Attack Severity Model
\ENSURE Adaptation actions based on detected attacks
\WHILE{system is operational}
\IF{$A$ is detected on $\mathcal{N}$ based on $\mathcal{M}$}
\STATE $AA \leftarrow$ AdaptationDecisionEngine($A$) from $tenant_n$
\IF{$AA \neq \text{Null}$}
\STATE $TLAA \leftarrow {aa \in AA \mid aa \text{ is a tenant-level adaptation action}}$
\STATE $MLAA \leftarrow {aa \in AA \mid aa \text{ is a middleware-level adaptation action}}$
\STATE TenantAdaptation($TLAA$) from $tenant_n$
\STATE MiddlewareAdaptation($MLAA$)
\ENDIF
\ENDIF
\ENDWHILE
\end{algorithmic}
\end{algorithm}

\begin{algorithm}
\caption{Service Monitoring Algorithm}
\label{alg:Service Monitoring Algorithm}
\begin{algorithmic}[1]
\REQUIRE $\mathcal{N}$: Real-time Network Traffic Data, $\mathcal{M}$: Trained Model for Attack Detection, $severity$: Attack Severity Model
\ENSURE Monitoring the Network Traffic Data
\WHILE{system is operational}
\IF{$A$ is detected on $\mathcal{N}$ based on $\mathcal{M}$}
\STATE $MLAA \leftarrow$ AdaptationDecisionEngine($A$) from $tenant_n$
\IF{$MLAA \neq \text{Null}$}
\STATE MiddlewareAdaptation($MLAA$)
\ENDIF
\ENDIF
\ENDWHILE
\end{algorithmic}
\end{algorithm}

==> Algorithms/draft.tex <==
\begin{algorithm}
\caption{Training Attack Detection Algorithm}
\begin{algorithmic} [1]
\REQUIRE $\mathcal{D}$: CLF+NTD
\ENSURE  $\mathcal{M}$: trained Random Forest model for attack detection
\STATE $\mathcal{D}{\text{train}}, \mathcal{D}{\text{test}} \gets$ Split($\mathcal{D}$) \Comment{ Split the dataset into training and testing sets}
\STATE $\mathcal{M} \gets$ TrainRandomForest($\mathcal{D}{\text{train}}$) \Comment{Train a Random Forest model on the training data}
\STATE$\text{Accuracy} \gets$ TestRandomForest($\mathcal{M}, \mathcal{D}{\text{test}}$) \Comment{Test the trained model on the testing data}
\STATE \Return $\mathcal{M}, \text{Accuracy}$ \Comment{Return the trained model and its accuracy}
\end{algorithmic}
\end{algorithm}


\begin{algorithm}
\caption{Attack Severity Learning with K-means and Chi-square}\label{alg:attack_severity_learning}
\begin{algorithmic}[1]
\REQUIRE{Dataset $\mathcal{D}$ with features $\mathcal{F}$}
\ENSURE{Attack severity model}
\STATE Perform chi-square feature selection on $\mathcal{D}$ to obtain feature subset $\mathcal{F'}$
\STATE Initialize K-means clustering with $K$ clusters
\STATE Initialize an empty dictionary $clusterDict$ to store the instances assigned to each cluster
\STATE Initialize an empty dictionary $severityDict$ to store the mean attack severity for each cluster
\STATE Randomly initialize the centroids for the $K$ clusters
\WHILE{not converged}
\FOR{each instance $x_i$ in $\mathcal{D}$}
\STATE Calculate the distance between $x_i$ and each centroid based on $\mathcal{F'}$
\STATE Assign $x_i$ to the cluster with the closest centroid
\ENDFOR
\STATE Update the centroids of the clusters by calculating the mean of the instances in each cluster
\ENDWHILE
\FOR{each cluster $c$}
\STATE Calculate the mean attack severity for the instances in $c$
\STATE Assign the mean attack severity to the cluster $c$ in $severityDict$
\ENDFOR
\STATE \textbf{return} $severityDict$
\end{algorithmic}
\end{algorithm}

==> Algorithms/formula.tex <==
\begin{align}
\text{Precision} &= \frac{TP}{TP + FP} 
\end{align}
\begin{align}
\text{Recall} &= \frac{TP}{TP + FN} \
\end{align}
\begin{align}
\text{F1-score} &= \frac{(1 + \beta^2) \cdot \text{recall} \cdot \text{precision}}{\beta^2 \cdot (\text{recall} + \text{precision})} \
\end{align}
\begin{align}
\text{Accuracy} &= \frac{TP + TN}{TP + TN + FP + FN} \
\end{align}
\begin{align}
\text{False Alarm Rate (FAR)} &= \frac{FP}{FP + TN}
\end{align}

==> Algorithms/name.tex <==
\begin{algorithm}
  \caption{Weighted Adaptation Action Prediction}\label{algorithm}
  \begin{algorithmic}[1]
    \REQUIRE
      \STATE $\text{Data} \gets \text{input dataset with features and adaptation actions}$
      \STATE $\text{weights} \gets \text{weight values for time, cost, value, mitigation score}$
      \STATE $\text{trainSet}, \text{testSet} \gets \text{splitData(Data)}$
    \ENSURE
      \STATE $\text{model} \gets \text{trained regression model}$
    \Procedure{WeightedPrediction}{$\text{model}, \text{weights}, \text{newInstance}$}
      \STATE $\text{prediction} \gets \text{model.predict(newInstance)}$
      \STATE $\text{weightedPrediction} \gets \text{0}$
      \FOR{$i \gets \text{0}$ \textbf{to} $\text{len(weights)}$}
        \STATE $\text{weightedPrediction} \gets \text{weightedPrediction} + (\text{prediction}[i] \times \text{weights}[i])$
      \ENDFOR
      \State \textbf{return} $\text{weightedPrediction}$
    \EndProcedure

    \Procedure{TrainModel}{$\text{trainSet}$}
      \STATE $\text{model} \gets \text{selected regression model}$
      \STATE $\text{model.train(trainSet)}$
      \STATE \textbf{return} $\text{model}$
    \EndProcedure

    \Procedure{EvaluateModel}{$\text{model}, \text{testSet}$}
      \STATE $\text{predictions} \gets \text{model.predict(testSet)}$
      \STATE $\text{metrics} \gets \text{calculateRegressionMetrics(testSet.adaptationActions, predictions)}$
      \STATE \textbf{return} $\text{metrics}$
    \EndProcedure

    \STATE $\text{trainSet}, \text{testSet} \gets \text{splitData(Data)}$
    \STATE $\text{model} \gets \text{TrainModel(trainSet)}$
    \STATE $\text{metrics} \gets \text{EvaluateModel(model, testSet)}$

    \STATE $\text{newInstance} \gets \text{new input instance}$
    \STATE $\text{weightedPrediction} \gets \text{WeightedPrediction(model, weights, newInstance)}$

    \STATE \textbf{print} $\text{"Regression Metrics: "} \text{metrics}$
    \STATE \textbf{print} $\text{"Weighted Prediction: "} \text{weightedPrediction}$
  \end{algorithmic}
\end{algorithm}



==> Sections/Motivation_Senario.tex <==
 \section{ Problem description and Motivation Scenario}
 To demonstrate the feasibility and significance of our approach, we developed a motivating example based on an insurance claim recovery chain (Figure \ref{figure_bpmnExample}). 
 \begin{figure}[bth!]
\includegraphics[width=\columnwidth]{figures/diagram_6.png}
\caption{Example Scenario}
\label{figure_bpmnExample}
\end{figure}
To demonstrate the feasibility and significance of our approach, we developed a motivating example based on an insurance claim recovery chain (Figure \ref{figure_bpmnExample}). This example serves as a use case to study the mitigation of security risks and costs associated with selected adaptations. The claim recovery process involves various tasks, starting with a customer submitting a claim recovery declaration to their insurance company, referred to as the tenant and the owner of the workflow. Upon receipt of the claim recovery declaration, the incident details service is promptly notified to retrieve relevant incident information. Following this, three parallel tasks are executed: requesting claim documents, hospital reports, and police reports, based on the obtained incident details. An expert then makes a reimbursement decision, triggering the Bank Reimbursement service if the claim is accepted. The customer is subsequently notified of the reimbursement decision, and finally, they are invited to provide feedback about the company and the overall process.

To address the security concerns specific to this example, we have defined specific security requirements for each task, including aspects such as integrity, confidentiality, and availability. Furthermore, Table \ref{Tenant Level Adaptation} outlines feasible adaptation actions at both the tenant and middleware levels for each task. Additionally, it presents the corresponding response time, price, and value relative to the original task's response time ($R$), price ($P$), and value ($V$). As observed in the table, the time and price for the "Rework" and "Redundancy" will be determined dynamically at runtime for all tasks, based on the selected backup service.  Also, for reconfiguration, the time, price, and value will be determined by their respective indexes ($T_{reconfig}$,  $P_{reconfig}$,  $V_{reconfig}$), set by the middleware.

 \begin{table*}[h!]
%\small
\fontsize{8pt}{10pt}\selectfont
\caption{{Tenant Level Adaptation} }
\label{Tenant Level Adaptation}
\def\arraystretch{1}
\ignorespaces 
%\centering 
\input{tables/table3}
\end{table*}

In our scenario, we assume the existence of 5 cloud providers, each offering 3 separate services. The service specifications are generated based on the ranges presented in Table \ref{Service-Specification}. Moreover, this paper specifically focuses on four prevalent types of attacks in cloud services and networks, namely Denial of Service (DoS), Remote-to-Local (R2L), User-to-Root (U2R), and probe attacks. The specifications of these attacks are provided in Table \ref{Attack-Specification}.

 \begin{table*}[h!]
%\small
\fontsize{8pt}{10pt}\selectfont
\caption{{Service Specifications} }
\label{Service-Specification}
\def\arraystretch{1}
\ignorespaces 
%\centering 
\input{tables/table5}
\end{table*}


 \begin{table*}[h!]
%\small
\fontsize{8pt}{10pt}\selectfont
\caption{{Attack Specifications} }
\label{Attack-Specification}
\def\arraystretch{1}
\ignorespaces 
%\centering 
\input{tables/table4}
\end{table*}
Also, we compute the normalized values of price, time, and value for different adaptation actions in Equation \ref{Equation:AdaptationCost}, using the following formula:

\begin{align}
AX_{normalized\underset{X \in \{P, T, V\}}{(aa)}} = \begin{cases}
AX_{aa} & \text{if } |finalAA| = 1 \\
0 & \text{if } |finalAA| > 1 \text{ and } maxX = minX \\
\frac{AX_{aa} - minX}{maxX - minX} & \text{if } |finalAA| > 1 \text{ and } maxX \neq minX \\
\end{cases}
\label{Equation:Normalized}
\end{align}


In Equation \ref{Equation:Normalized}, X can represent the price, time, or value for a specific adaptation action $aa$. The variables $maxX$ and $minX$ correspond to the maximum and minimum values among the adaptation options for the respective X. The formula considers three scenarios: a)If there is only one adaptation action ($|finalAA| = 1$), no normalization is needed, and the original value, denoted as $AX_{aa}$, is used. b) If there are multiple adaptation actions and the maximum and minimum values are the same ($maxX = minX$), indicating equal values for all options, the normalized value is set to 0. c) For multiple adaptation actions with different maximum and minimum values ($maxX \neq minX$), the normalized value is calculated as $\frac{AX_{aa} - minX}{maxX - minX}$.




The given formula represents the process of calculating the normalized values for the price, time, and value of different adaptation actions. This calculation is performed in Equation \ref{Equation:Normalized}, which builds upon the concepts introduced in Equation \ref{Equation:AdaptationCost}.

In Equation \ref{Equation:Normalized}, the variable $AX_{normalized\underset{X \in {P, T, V}}{(aa)}}$ represents the normalized value of a specific factor (price, time, or value) for an adaptation action $aa$. The subscript $X \in {P, T, V}$ indicates that $X$ can take on values from the set ${P, T, V}$, which corresponds to the factors of price, time, and value.

The formula within the cases environment specifies three different cases for calculating the normalized value, depending on the conditions:

If there is only one adaptation action available for the detected attack, indicated by $|finalAA| = 1$, there is no need for normalization. In this case, the normalized value remains the same as the original value ($AX_{aa}$).

If there are multiple adaptation actions ($|finalAA| > 1$) and the maximum and minimum values of the factor are equal ($maxX = minX$), it implies that all adaptation options have the same value for that factor. In such cases, the normalized value is set to 0.

If there are multiple adaptation actions ($|finalAA| > 1$) and the maximum and minimum values of the factor are different ($maxX \neq minX$), the normalized value is calculated by subtracting the minimum value ($minX$) from the original value ($AX_{aa}$) and dividing the result by the range of values ($maxX - minX$). This normalization process scales the values between 0 and 1.

The explanation further clarifies that in Equation \ref{Equation:Normalized}, the variable $X$ can represent the price, time, or value for the adaptation action $aa$. The variables $maxX$ and $minX$ correspond to the maximum and minimum amounts for the respective factor (price, time, or value). The conditions $|finalAA| = 1$ and $maxX = minX$ are used to handle specific scenarios and ensure appropriate normalization when necessary.

\subsection{Main Results}
 In this section, we described our settings for different parts of the experiments. In this paper, we specifically focused on four prevalent types of attacks in cloud services and networks including Denial of Service (DoS), Remote-to-Local (R2L), User-to-Root (U2R), and probe attacks.
 We evaluated the proposed solution using multiple workflow models, each consisting of different numbers of service tasks and exhibiting various control and data dependencies. Our evaluation focused on the following key aspects:

Attack Detection: We measured the accuracy and efficiency of the attack detection module in identifying security violations during workflow execution. This evaluation provided insights into the system's ability to detect attacks in real-time and mitigate their impact.

Adaptation Effectiveness: We assessed the effectiveness of the adaptation module in selecting and executing appropriate adaptation actions to mitigate the impact of detected attacks. This evaluation considered factors such as the reduction in attack severity, resource utilization, and workflow performance.

Scalability: We examined the scalability of the proposed solution by varying the size and complexity of the workflow models. This evaluation aimed to determine the system's performance and resource requirements as the workload and number of tasks increased.

Comparative Analysis: We compared the performance of the proposed solution against existing methods or alternative approaches in terms of attack detection accuracy, adaptation effectiveness, and overall system performance. This analysis provided insights into the advantages and limitations of our solution compared to other techniques.

We present the detailed experimental results and analysis in the following section.


==> Sections/Proposed_Detection_method-randomForest.tex <==
\section{Proposed solution}
\label{sec:Proposed solution}
In this section, we introduce our proposed monitoring and detection system, specifically designed to identify security violations occurring during the execution of workflows in both network and cloud services. It is important to emphasize that, while our previous section presented a comprehensive system, here we primarily focus on addressing the monitoring and detection aspects specifically associated with the cloud and its related services. The investigation of other types of attackers, as described in the previous section, will be a subject of future research since they extend beyond the scope of this paper. 

To establish a clear understanding of the key concepts involved, we begin this section by introducing important definitions. These definitions serve as the foundation for subsequent formulas and explanations, ensuring a solid comprehension of the proposed solution. Furthermore, we provide a comprehensive description of the proposed solution, outlining its key components and methodologies.

%\input{tables/table2}
\textbf{Definition 1 (Task)}: A task $t$ represents a service task that utilizes a cloud service for execution. It is defined as a tuple ($C$, $I$, $A$, $V$, $AA$), where $C$, $I$, and $A$ represent the Confidentiality, Integrity, and Availability requirements of task $t$, respectively. Additionally, $V$ indicates the Value of this task within the overall workflow. Moreover, $AA$ indicates a set of feasible Adaptation Actions for task $t_i$, which can include a combination of actions from both Tenant Adaptation Actions ($TAA$) and Middleware Adaptation Actions ($MAA$). Mathematically, this set can be represented as $AA = \{aa \mid aa \in TAA_{t_i} \cup MAA_{t_i}\}$.

\textbf{Definition 2 (Tenant Adaptation Action)}: Tenant Adaptation Actions ($TAA_{t_i}$) refers to the actions that can be taken to minimize the damage caused by a violation in task $t$. Each of these actions denoted as $Taa_{t_i}$ is defined as a tuple ($P$, $T$, $MS$, $V$) that represents the Price, Time, Mitigation Score, and overall Value of the adaptation action in task $t$ for the workflow. These parameters are determined during the workflow modeling phase, considering the specific characteristics and requirements of each action in the task.

\textbf{Definition 3 (Middleware Adaptation Action)}: Middleware Adaptation Actions ($MAA_{t_i}$) represents the actions that can be employed at the middleware level to minimize the damage caused by a violation in task $t$. Each of these actions denoted as $Maa_{t_i}$ is defined as a tuple ($P$, $T$, $MS$, $V$) that indicates the Price, Time, Mitigation Score, and overall Value of the adaptation action in task $t$ for the workflow. As the middleware-level adaptation depends on execution time and the availability of cloud services, these parameters cannot be pre-defined during the modeling phase; rather, they are established dynamically at runtime when an attack occurs, serving as the backup service.

\textbf{Definition 4 (Workflow)}: A Workflow, $w$, is a tuple ($ST$, $D$, $E_c$, $E_d$) where ST is a set of service tasks $t$, D is the set of data, $E_c$ is a set of control edges that define the order in which the tasks are performed based on the set of conditions that must be met  $E_c \subset ST\times ST\times Conds(D)$, $E_d$ is a set of data edges that specify the flow of data between the tasks $E_d \subset ST\times ST\times D$.

\textbf{Definition 5 (Attack)}: An attack $a$ refers to a security violation that can potentially occur during the execution of a workflow $W$ at task $t$, compromising the security of the task that utilizes service $s$. It is defined as a tuple ($C$, $I$, $A$, $AT$, $MA_{H}$, $MA_{M}$, $MA_{L}$), where $C$, $I$, and $A$ represent the impacts of the attack $a$ on Confidentiality, Integrity, and Availability, respectively. The variable $AT$ denotes the Attack Type. Additionally, mitigation actions are available to minimize the impact of the attack and are categorized into three levels: $MA_{H}$, $MA_{M}$, and $MA_{L}$. These levels correspond to High, Medium, and Low severity levels of actions that can be taken to mitigate the impact of the attack, respectively.

\textbf{Definition 6 (Service)}: A service $s$ represents the service provided by the provider $p$. It is defined as a tuple ($P$, $T$, $C$, $I$, $A$, $AFR$), where $P$ and $T$ indicate the Price and average response Time of the service, respectively. Furthermore, $C$, $I$, and $A$ denote the levels of Confidentiality, Integrity, and Availability offered by the service, respectively. Additionally, $AFR$ represents the Attack Frequency Rate of service $s$ for different types of attacks. The Attack Frequency Rate is represented as $AFR = \bigcup_{AT \in \text{all AttackTypes}} AFR(AT)$, which reflects the likelihood of each attack type occurring within the service based on historical data.

\subsection{Service and Network Model Trainer}
This section provides an overview of the training phase for the attack detection model, utilizing the Random Forest and Linear Regression machine learning algorithms. The primary objective of this algorithm is to train a robust model capable of effectively detecting attacks. A comparison is made between these two methods to evaluate their performance.

To achieve this objective, we present a high-level overview of the training algorithm in Algorithm \ref{alg:TraininAttackDetectiongAlgorithm}. The algorithm utilizes two distinct datasets: the Network Traffic Data (NTD) and the Cloud Log File (CLF).

The NTD dataset contains historical records of network traffic data exchanged between the middleware and cloud services. It serves as the foundation for identifying potential network attacks. On the other hand, the CLF dataset comprises the cloud log file, which provides information about the utilization of resources such as RAM, CPU, and Bandwidth during the execution of various services. This dataset is employed for detecting attacks that specifically target the services.

Furthermore, Algorithm \ref{alg:attack_severity_learning} introduces an algorithm designed to learn the attack severity model for multiple attack types. This algorithm employs K-means clustering and chi-square feature selection techniques to assign a severity level to each attack. It takes into account the distinctive features of each attack type to accurately score their severity. The Chi-Square Feature Selection is applied to identify the most informative features for each attack type. This ensures that the severity scoring incorporates the specific characteristics and patterns associated with different types of attacks. By considering different features for each attack type, the algorithm significantly enhances the accuracy and granularity of the severity assignment.

\subsection{Adaptation Model Trainer}
In this section, we utilize the random forests algorithm to train a model for selecting adaptation actions. The training process involves generating a dataset through simulations, encompassing various attacks with different severity levels in different tasks of workflows under diverse scenarios. The dataset incorporates crucial information such as randomly selected actions for attacks, final execution times, prices, values, and mitigation scores for the entire workflow execution. By considering these features collectively, the algorithm trains an initial model to select the optimal adaptation action for a detected attack with a specific severity. Subsequently, the model is periodically updated and refined based on new data obtained from system reactions, particularly from the Adaptation Decision Engine, and the impact of these actions on the system.


\input{Algorithms/Training Attack Detection Model-NTD}
\input{Algorithms/Attack Severity }
\input{Algorithms/Training Action Selection}

\subsection{Service Monitoring}
The service monitoring module plays a crucial role in the real-time detection of service attacks using data obtained from various sources, including the real-time service information file and network traffic data. An overview of the monitoring procedure can be found in Algorithm \ref{alg:Service Monitoring Algorithm}.

To identify potential attacks ($a_k$), the algorithm leverages the trained model for attack detection ($\mathcal{M}$) to analyze the real-time data. When an attack is detected, the severity of the attack is calculated based on Algorithm \ref{alg:attack_severity_learning}. Subsequently, considering the possibility of re-work as a viable option within the middleware level adaptation actions ($MAA_{t_i}$), the algorithm searches for a suitable backup service for $t_i$ denoted as $BackupSrc_{t_i}$. It calculates the parameters $P$, $T$, $MS$, and $V$ associated with this backup service, taking into account the available cloud service offerings. Finally, the algorithm proceeds to the adaptation decision module of the relevant tenant ($relatedTenant$).
\input{Algorithms/Service Monitoring Algorithm}

\subsection{Adaptation Decision Engine}
In this section, we present the Adaptation Decision Engine, which plays a crucial role in dynamically identifying the most suitable adaptation actions to mitigate the impact of attacks on the workflow. This engine utilizes the Adaptation Action Selection algorithm (Algorithm \ref{alg:Adaptation Action Selection Algorithm}) to make informed decisions.
\input{Algorithms/Adaptation Action Selection Algorithm }

The Adaptation Action Selection algorithm begins by computing the attack score, which quantifies the severity of the current attack on the task using Equation \ref{eq:attack_score}. If the attack score surpasses the pre-defined Adaptation Trigger Threshold ($Tenant.AdaptTriggerThresh$), the algorithm proceeds with the adaptation action selection process.

Two distinct strategies are employed to select the optimal adaptation action: the Lowest-Cost Strategy and the Predictive Strategy.

The Lowest-Cost Strategy initially identifies a set of potential adaptation actions, denoted as $finalAA$. This set is determined by intersecting the mitigation actions suitable for the severity of the detected attack ($MA_{l_{(a_k)}}$) and the feasible adaptation actions for the current task ($AA_{t_i}$). The potential actions are then evaluated based on factors such as price, time, mitigation score, and overall value, computed using Equation \ref{eq:AdaptationCost} with assigned weights for each workflow. The actions are subsequently sorted based on their computed costs, and the one with the lowest cost is selected as the optimal choice for mitigating the attack. 

Furthermore, to address the uncertainty of the cost associated with each action in the adapted task and its impact on other tasks within the workflow, we propose the implementation of an additional strategy called the Predictive Strategy. This strategy utilizes a model trained using Algorithm \ref{alg:Adaptation Action Selection Algorithm}, which leverages historical system reactions and adaptations to violations. This trained model is capable of predicting the most optimal adaptation action. Periodic updates to the model are made based on recent system reactions, ensuring its responsiveness to evolving conditions. By incorporating this approach, we are able to consider the dynamic consequences and costs associated with each action. These consequences cannot be statically determined at the time of selecting the adaptation action to respond to the attack. Moreover, our consideration extends beyond the task in which the attack is detected, encompassing the entire workflow. By taking a holistic view of the situation, including any violations occurring in other tasks that may impact the selection of the best adaptation action for the current task, we are able to properly assess the overall scenario. This comprehensive assessment enables us to make informed decisions regarding the appropriate adaptation action. The predictive model we have developed provides valuable insights, incorporating past reactions and adaptations to violations. These insights enhance the decision-making process and support effective responses to attacks.

After the selection of the adaptation action(s), the algorithm determines whether they belong to the tenant-level actions or the middleware-level actions. If the action(s) falls under the tenant-level category, the Tenant Adaptation module is invoked to initiate the necessary adaptations at the tenant level. Conversely, if the action(s) are categorized as middleware-level adaptations, the Middleware Adaptation module is called upon to implement the required changes.

\subsubsection{Compute The Attack Score}
The attack Score serves as a crucial metric for evaluating the impact of the attack detected in the cloud services (current service) used by the current task in the workflow. It plays a vital role in subsequent stages of the adaptation process, guiding the selection of appropriate adaptation actions to mitigate the attack's impact on the workflow effectively. The Attack Score is calculated using the following equation:

\begin{align} \label{eq:attack_score}
   AttackScore(a_k,t_i,s_j,l_{a_k})= (1 -\prod_{obj \in \{CIA\}} (1 - obj_{t_i} \cdot obj_{a_k})) \cdot AFR_{s_j}(AT_{a_k}) \cdot l_{a_k}
\end{align} 

In this equation, $obj_{t_i}$ represents the security requirement of the current task $t_i$ in the workflow for each security objective (CIA, including confidentiality, integrity, and availability). $obj_{a_k}$ denotes the security impact of the detected attack $a_k$ on each security objective. $AFR_{s_j}(AT_{a_k})$ represents the Attack Frequency Rate (AFR) in the cloud service $s_j$ for the type of detected attack $AT_{a_k}$. Lastly, $l_{a_k}$ corresponds to the severity of the detected attack $a_k$ learned by the algorithm \ref{alg:attack_severity_learning}. 


\subsubsection{Compute The Adaptation Cost}
The Adaptation Cost is a metric used to score all possible adaptation actions aimed at mitigating the detected attack. It plays a critical role in Adaptation Decision Engine by enabling effective evaluation and comparison of the available actions based on the tenant's preferences. It takes into account various parameters, such as price, time, mitigation score, and value. In simpler terms, it calculates these parameters for each adaptation action and then computes the final adaptation cost for it, considering the weight assigned to each parameter by the tenant. To achieve this, we assess the potential impact of an adaptation action on the overall workflow for each parameter. This is accomplished by quantifying the change or impact that the adaptation action may introduce to each parameter. This is achieved by determining the extent of modification or adjustment that can be expected in each parameter as a result of adopting the adaptation action. Subsequently, we determine the final adaptation cost by employing Equation \ref{eq:AdaptationCost}. 
\begin{align}
\begin{split}
AdaptationCost(aa) &= W_{Price} \cdot P_{normalized}(aa) + W_{Time} \cdot T_{normalized}(aa)- \\
&\quad W_{Security} \cdot MS_{normalized}(aa) - W_{Value} \cdot V_{normalized}(aa)
\end{split}
\label{eq:AdaptationCost}
\end{align}
In Equation \ref{eq:AdaptationCost}, the terms $W_{Price}$, $W_{Time}$, $W_{Security}$, and $W_{Value}$ represent the weights assigned by the tenant to price, time, security, and value, respectively, for the given workflow. On the other hand, $P_{normalized}(aa)$, $T_{normalized}(aa)$,  $MS_{normalized}(aa)$, and $V_{normalized}(aa)$ denote the normalized price, time, mitigation score, and value, respectively, for the adaptation action $aa$. The time, price, and value are directly assigned based on the adaptation type, while the mitigation score is calculated using Equation \ref{Equation:MitigationScore}. This equation takes into consideration the security requirements of task $t$ (represented by $obj_t$), the impact of the detected attack $a_i$ on the confidentiality, integrity, and availability (CIA) aspects (represented by $obj_{a_i}$), and the mitigation impact of the adaptation action on each aspect (represented by $obj_{MI_{aa}}$).

\begin{align}
MitigationScore(aa,t,a_i) = \sum_{obj \in {C,I,A}} (1 - obj_t \cdot obj_{a_i}) \cdot obj_{MI_{aa}}
\label{Equation:MitigationScore}
\end{align}













==> Sections/Proposed_Detection_method.tex <==
\section{Proposed solution}
\label{sec:Proposed solution}
In this section, we introduce our proposed monitoring and detection system, specifically designed to identify security violations occurring during the execution of workflows in both network and cloud services. It is important to emphasize that, while our previous section presented a comprehensive system, here we primarily focus on addressing the monitoring and detection aspects specifically associated with the cloud and its related services. The investigation of other types of attackers, as described in the previous section, will be a subject of future research since they extend beyond the scope of this paper. 

To establish a clear understanding of the key concepts involved, we begin this section by introducing important definitions. These definitions serve as the foundation for subsequent formulas and explanations, ensuring a solid comprehension of the proposed solution. Furthermore, we provide a comprehensive description of the proposed solution, outlining its key components and methodologies.

%\input{tables/table2}
\textbf{Definition 1 (Task)}: A task $t$ represents a service task that utilizes a cloud service for execution. It is defined as a tuple ($C$, $I$, $A$, $V$, $AA$), where $C$, $I$, and $A$ represent the Confidentiality, Integrity, and Availability requirements of task $t$, respectively. Additionally, $V$ indicates the Value of this task within the overall workflow. Moreover, $AA$ indicates a set of feasible Adaptation Actions for task $t_i$, which can include a combination of actions from both Tenant Adaptation Actions ($TAA$) and Middleware Adaptation Actions ($MAA$). Mathematically, this set can be represented as $AA = \{aa \mid aa \in TAA_{t_i} \cup MAA_{t_i}\}$.

\textbf{Definition 2 (Tenant Adaptation Action)}: Tenant Adaptation Actions ($TAA_{t_i}$) refers to the actions that can be taken to minimize the damage caused by a violation in task $t$. Each of these actions denoted as $Taa_{t_i}$ is defined as a tuple ($P$, $T$, $MS$, $V$) that represents the Price, Time, Mitigation Score, and overall Value of the adaptation action in task $t$ for the workflow. These parameters are determined during the workflow modeling phase, considering the specific characteristics and requirements of each action in the task.

\textbf{Definition 3 (Middleware Adaptation Action)}: Middleware Adaptation Actions ($MAA_{t_i}$) represents the actions that can be employed at the middleware level to minimize the damage caused by a violation in task $t$. Each of these actions denoted as $Maa_{t_i}$ is defined as a tuple ($P$, $T$, $MS$, $V$) that indicates the Price, Time, Mitigation Score, and overall Value of the adaptation action in task $t$ for the workflow. As the middleware-level adaptation depends on execution time and the availability of cloud services, these parameters cannot be pre-defined during the modeling phase; rather, they are established dynamically at runtime when an attack occurs, serving as the backup service.

\textbf{Definition 4 (Workflow)}: A Workflow, $w$, is a tuple ($ST$, $D$, $E_c$, $E_d$) where ST is a set of service tasks $t$, D is the set of data, $E_c$ is a set of control edges that define the order in which the tasks are performed based on the set of conditions that must be met  $E_c \subset ST\times ST\times Conds(D)$, $E_d$ is a set of data edges that specify the flow of data between the tasks $E_d \subset ST\times ST\times D$.

\textbf{Definition 5 (Attack)}: An attack $a$ refers to a security violation that can potentially occur during the execution of a workflow $W$ at task $t$, compromising the security of the task that utilizes service $s$. It is defined as a tuple ($C$, $I$, $A$, $AT$, $MA_{H}$, $MA_{M}$, $MA_{L}$), where $C$, $I$, and $A$ represent the impacts of the attack $a$ on Confidentiality, Integrity, and Availability, respectively. The variable $AT$ denotes the Attack Type. Additionally, mitigation actions are available to minimize the impact of the attack and are categorized into three levels: $MA_{H}$, $MA_{M}$, and $MA_{L}$. These levels correspond to High, Medium, and Low severity levels of actions that can be taken to mitigate the impact of the attack, respectively.

\textbf{Definition 6 (Service)}: A service $s$ represents the service provided by the provider $p$. It is defined as a tuple ($P$, $T$, $C$, $I$, $A$, $AFR$), where $P$ and $T$ indicate the Price and average response Time of the service, respectively. Furthermore, $C$, $I$, and $A$ denote the levels of Confidentiality, Integrity, and Availability offered by the service, respectively. Additionally, $AFR$ represents the Attack Frequency Rate of service $s$ for different types of attacks. The Attack Frequency Rate is represented as $AFR = \bigcup_{AT \in \text{all AttackTypes}} AFR(AT)$, which reflects the likelihood of each attack type occurring within the service based on historical data.


\subsection{Training Attack Detection Model}
This section provides an overview of the training phase for the attack detection model, which utilizes the Random Forest machine learning algorithm. The primary objective of this algorithm is to train a robust model that can effectively detect attacks. To accomplish this, the algorithm leverages two distinct datasets: the Network Traffic Data (NTD) and the Cloud Log File (CLF).

The NTD dataset contains historical records of network traffic data exchanged between the middleware and cloud services. It serves as the basis for detecting potential network attacks. On the other hand, the CLF dataset comprises the cloud log file, which includes information on the utilization of resources such as RAM, CPU, and network during the execution of various services. This dataset is utilized for detecting attacks specifically targeting the services.

Algorithm \ref{alg:TrainingAlgorithm} provides a high-level overview of the training process, outlining the steps involved in training the attack detection model using the NTD and CLF datasets.
%\input{Algorithms/Training Attack Detection Model}
\input{Algorithms/Training Attack Detection Model-NTD}

In addition, Algorithm \ref{alg:attack_severity_learning} presents an algorithm for learning the attack severity model for multiple attack types using K-means clustering and chi-square feature selection. 
\input{Algorithms/Attack Severity }

\subsection{Service monitoring}
The service monitoring module plays a crucial role in the real-time detection of service attacks using data obtained from various sources, including the real-time service information file and network traffic data. An overview of the monitoring procedure can be found in Algorithm \ref{alg:Service Monitoring Algorithm}.

To identify potential attacks ($a_k$), the algorithm leverages the trained model for attack detection ($\mathcal{M}$) to analyze the real-time data. When an attack is detected, the severity of the attack is calculated based on Algorithm \ref{alg:attack_severity_learning}. Subsequently, considering the possibility of re-work as a viable option within the middleware level adaptation actions ($MAA_{t_i}$), the algorithm searches for a suitable backup service for $t_i$ denoted as $BackupSrc_{t_i}$. It calculates the parameters $P$, $T$, $MS$, and $V$ associated with this backup service, taking into account the available cloud service offerings. Finally, the algorithm proceeds to the adaptation decision module of the relevant tenant ($relatedTenant$).
\input{Algorithms/Service Monitoring Algorithm}

\subsection{Adaptation Decision Engine}
In this section, we introduce the Adaptation Action Selection algorithm \ref{alg:Adaptation Action Selection Algorithm}, which plays a crucial role in dynamically identifying the most suitable adaptation actions to mitigate the impact of attacks on the entire workflow. The algorithm initiates by computing the attack score through Equation \ref{eq:attack_score}, which effectively quantifies the severity of the attack on the current task. Subsequently, the algorithm proceeds with the adaptation action selection if the attack score surpasses the pre-established Adaptation Trigger Threshold defined by the tenant, represented as $Tenant.AdaptTriggerThresh$.
 \input{Algorithms/Adaptation Action Selection Algorithm }

Then, the algorithm proceeds to identify a set of potential adaptation actions, denoted as $finalAA$. This set is determined by intersecting the attack mitigation actions suitable for the severity of the detected attack ($MA_{l_{(a_k)}}$) and the feasible adaptation actions for the current task ($AA_{t_i}$), resulting in a collection of actions that are both applicable to the task $t_i$ and capable of mitigating the impact of detected attack $a_k$. The cost of each potential action is then calculated using Equation 2, which takes into account various factors such as price, time, mitigation impact, and the overall value it brings to the entire workflow. These factors collectively assess the feasibility and effectiveness of each action. Subsequently, the potential actions are sorted in ascending order based on their computed costs.

Next, the algorithm selects the adaptation action with the lowest cost as the optimal choice for mitigating the attack. It's important to note that the tenant's adaptation decision strategy may influence this selection. For instance, to achieve greater mitigation of the attack impact, a combination of adaptation actions from both tenant and middleware levels may be chosen, instead of a single action.

Once the adaptation action(s) is selected, the algorithm determines whether it belongs to the tenant-level actions or the middleware-level actions. If it falls under the category of tenant-level actions, the Tenant Adaptation module is invoked to initiate the required adaptations at the tenant level. Conversely, if the action(s) is categorized as a middleware-level adaptation, the Middleware Adaptation module is called upon to implement the necessary changes.

\subsubsection{Compute The Attack Score}
The attack Score serves as a crucial metric for evaluating the impact of the attack detected in the cloud services (current service) used by the current task in the workflow. It plays a vital role in subsequent stages of the adaptation process, guiding the selection of appropriate adaptation actions to mitigate the attack's impact on the workflow effectively. The Attack Score is calculated using the following equation:

\begin{align} \label{eq:attack_score}
   AttackScore(a_k,t_i,s_j,l_{a_k})= (1 -\prod_{obj \in \{CIA\}} (1 - obj_{t_i} \cdot obj_{a_k})) \cdot AFR_{s_j}(AT_{a_k}) \cdot l_{a_k}
\end{align} 

In this equation, $obj_{t_i}$ represents the security requirement of the current task $t_i$ in the workflow for each security objective (CIA, including confidentiality, integrity, and availability). $obj_{a_k}$ denotes the security impact of the detected attack $a_k$ on each security objective. $AFR_{s_j}(AT_{a_k})$ represents the Attack Frequency Rate (AFR) in the cloud service $s_j$ for the type of detected attack $AT_{a_k}$. Lastly, $l_{a_k}$ corresponds to the severity of the detected attack $a_k$ learned by the algorithm \ref{alg:attack_severity_learning}. 

\subsubsection{Compute The Adaptation Cost}
The Adaptation Cost is a metric used to score all possible adaptation actions aimed at mitigating the detected attack. It plays a critical role in Adaptation Decision Engine by enabling effective evaluation and comparison of the available actions based on the tenant's preferences. It takes into account various parameters, such as price, time, mitigation score, and value. In simpler terms, it calculates these parameters for each adaptation action and then computes the final adaptation cost for it, considering the weight assigned to each parameter by the tenant. To achieve this, we assess the potential impact of an adaptation action on the overall workflow for each parameter. This is accomplished by quantifying the change or impact that the adaptation action may introduce to each parameter. This is achieved by determining the extent of modification or adjustment that can be expected in each parameter as a result of adopting the adaptation action. Subsequently, we determine the final adaptation cost by employing Equation \ref{eq:AdaptationCost}. 
\begin{align}
\begin{split}
AdaptationCost(aa) &= W_{Price} \cdot P_{normalized}(aa) + W_{Time} \cdot T_{normalized}(aa)- \\
&\quad W_{Security} \cdot MS_{normalized}(aa) - W_{Value} \cdot V_{normalized}(aa)
\end{split}
\label{eq:AdaptationCost}
\end{align}
In Equation \ref{eq:AdaptationCost}, the terms $W_{Price}$, $W_{Time}$, $W_{Security}$, and $W_{Value}$ represent the weights assigned by the tenant to price, time, security, and value, respectively, for the given workflow. On the other hand, $P_{normalized}(aa)$, $T_{normalized}(aa)$,  $MS_{normalized}(aa)$, and $V_{normalized}(aa)$ denote the normalized price, time, mitigation score, and value, respectively, for the adaptation action $aa$.













==> Sections/Security_Evaluator.tex <==
\section{Security Evaluator}

Propagation Patterns
Goal: Describe the propagation of different violation to the other tasks in the workflow.
For: different security objectives(Confidentiality, Integrity, Availability)
How to Calculate: Considering one task or data is under attack, then measure the effect of this vulnerability on the other tasks/data. 
Usage: Prevent propagation of the attacks to the other tasks after detecting any violation. 
Separation Patterns 


Security-aware Scheduling based on these patterns 
rkflows in order to prevent clouds from inferring more undisclosed privacy information and the relationship between the results through analysis of the collected data (data/logic confidentiality violation).

Goal: Describe which tasks from which instances should be deployed in the separate clouds. 
Prevent Clouds from combing the data from different workflow tasks or fragments to one instace : If one cloud has two or more tasks/fragments of one instance, it can infer additional privacy information by combining multiple pieces of such data.
Prevent Clouds from combing the data from different workflow instances belonging to one user/tenant: If one cloud has all instances related to the one entity, it can infer some sensitive information about it.
For: Instance/User/Tenant separation)
How to Calculate: find the sensitive tasks, find the number of different cases necessary to mine a BP model,… 
Usage: Security-aware Scheduling based on these patterns 
Security-aware scheduler
Tenant’s Workflow Monitoring module 


1-2-2- Confidentiality Requirements model
in the Confidentiality Evaluator phase, we define  a set of the Confidentiality Requirements for each workflow. 
Definition 1 (Instance Separation Pattern). This separation pattern shows the confidentiality relationship between tasks in one instance. In other words, it expresses if one cloud has two or more tasks of one instance, it can infer additional privacy information by combining multiple pieces of such data. This pattern is represented as a t*t-dimensional matrix (t = |Tasks |), where 〖SP〗_instance[i][j]=1 (i,j∈Tasks) indicates whether  t_i   and t_j shouldn’t assign to same cloud provider.
〖SP〗_instance [i][j]={█(1       t_i  ,t_j  shouldn’t assign to the same cloud @0                           no restriction between t_i,t_j  )┤

Example 1. The follow example shows the propagation pattern of the motivation scenario. As the ”initiate claim” task includes the private data from the customer (like name, address, bank account info, and etc.), the customer’s identity should be anonymized in the task’s output data, otherwise the confidentiality degree of this data will be propagate to the all following tasks. This matrix indicates that t_0 shouldn’t be located at the same cloud with the other tasks as all of the referred values are 1. Also, as there is no other restriction for the further tasks, the other values are 0.
                                    ■(t_0&t_1&t_2&t_3&t_4&t_5&t_6 )
P_Propagation=■(t_0@t_1@t_2@t_3@t_4@t_5@t_6 ) [■(0&1&1&1&1&1&1@1&0&0&0&0&0&0@1&0&0&0&0&0&0@1&0&0&0&0&0&0@1&0&0&0&0&0&0@1&0&0&0&0&0&0@1&0&0&0&0&0&0) ]


Definition 2 (User Separation Pattern). This pattern preserves the confidentiality of the users involved in the workflow by preventing a single cloud from executing all critical tasks related to a user. This pattern is represented as a t*u-dimensional matrix (u = |Users |) , where 〖SP〗_user[i][j]=v (i∈Tasks,j∈Users) indicates the maximum number of t_i tasks from different instances belonging to the u_j that can be assigned to one cloud provider. 

                                   


Example 2. In the motivation scenario, there are four users involved in the instances: Client, Police, Hospital, and Expert. As an example, if one cloud has all instances related to the one client, it can infer number of her/his accident, history of her/his medical treatment, etc. So, based on the separation rate, we can define the maximum number of allowed instances of each user assigned to one cloud in the specific time  period.
                         ■(t_0   &t_1& t_2& t_3&〖 t〗_4& t_5& t_6 )
〖SP〗_user=■(u_0@u_1@u_2@u_3 ) [■(3&0&0&0&0&0&3@0&0&10&0&0&0&0@0&0&0&20&0&0&0@0&0&0&0&5&0&0) ]

Definition 3 (Tenant Separation Pattern). This pattern try to preserve the data and logic privacy of each tenant by preventing a single cloud from executing all critical tasks related to a tenant. This pattern is represented as a t-dimensional matrix, where 〖SP〗_tenant [i]=1 (i∈Tasks) indicates that the set of t_i   tasks from different instances belonging to one tenant shouldn’t assign to one cloud provider. Also, r_seperation is a m-dimensional matrix (m = |Tenants |)  where r_seperation [k]=v (k∈Tenants) and v shows the maximum number of tasks from different instances belonging to tenant k that can be assigned to one cloud provider.

                                   


Example 2. In the motivation scenario, if one cloud has all instances related to one tenant (insurance company), it can infer the information like the number of its clients and their specifications, the total amounts and taxes, etc. So, based on the separation rate, we can define the maximum number of allowed instances of each tenant assigned to one cloud in the specific time period.
                                ■(t_0&t_1&t_2&t_3&t_4&t_5&t_6 )
                                                〖SP〗_tenant= [■(1&0&0&0&0&0&1) ]

                                 ■(〖tenant〗_(0  )  &〖tenant〗_(1 )  &〖tenant〗_2 )
 		 		r_seperation= [■(10       &12           &6) ]


Definition 3 (Attack Propagation Pattern). 



Example 2 :From the motivation example




==> Sections/System_Architecture_and_Motivation_Scenario.tex <==
  \section{System Architecture and Design}
  In the following, first, we present a motivation scenario to provide some clear examples to explain the problem and our proposed solution. Then, The system model 

\subsection{System Architecture}
This section outlines the proposed architecture of our security-aware Workflow Management System (WFMS) to ensure that workflows are protected from security violations throughout their lifecycle (see Figure \ref{figure_Architecture}).
\begin{figure*}[h]
  \includegraphics[width=\textwidth]{figures/Architecture1.1.pdf}
  \caption{The Proposed Security-aware WFMS}
  \label{figure_Architecture}
\end{figure*}
 \subsection{Tenant’s Kernel}
\label{Tenant’s Kernel}
 The Tenant's Kernel provides an isolated environment for each tenant where they can model, analyze and adapt workflows based on their requirements and strategies. This ensures that the decisions and data of one tenant are protected from other tenants. It consists of the following four sub-modules. 

\subsubsection{Workflow Modeller}
\label{Section:Security Modeller}
The Workflow Modeller module enables tenants to model their workflows in a secure and efficient way. During the modeling process, the security requirements (confidentiality, integrity, and availability) of each task are defined. 

\subsubsection{Security Evaluator}
\label{Section:Security Evaluator}
 In this module, the possible adaptation actions for each task are defined here. This requires establishing a set of adaptation strategies (e.g., skipping, re-working, re-sequencing, re-configuration) for each task in the workflow model and determining their potential impact on the overall value of the workflow and on the balance between value and security properties. As an example of such specification, consider the scenario of skipping certain tasks within the workflow, some tasks may be less critical, and skipping them may have little impact on the overall workflow value. However, for other tasks, such as authentication tasks, skipping is not even an option in case of any violation, as they are essential to the security of the workflow. In such cases, the impact of skipping could be significant and compromise the overall security of the workflow. Therefore, by incorporating such specifications for each task in the security evaluator module after the modeling phase, the cost of each adaptation action could be estimated in execution time, thus allowing to select the most viable adaptation option for any violations that may arise. 

\subsubsection{Task Anonymizer }
\label{Section:Task Anonymizer}
This module is responsible for handling sensitive input data in a secure and efficient manner in a cloud computing environment. To achieve this, it utilizes appropriate obfuscation techniques to anonymize sensitive information before submitting tasks to the navigator for scheduling and allocation to the planned cloud services and resources for execution. This sensitive information for each task includes all unnecessary information for processing that task such as Workflow-ID, Instance-ID, names, addresses, etc. After execution, this obfuscated information is included in the intermediate results for upcoming tasks, if needed. It utilizes appropriate obfuscation techniques such as tokenization and salting to ensure the security of sensitive data. Tokenization involves replacing sensitive data with a unique identifier or token, while salting involves adding a random string of characters to the sensitive data before hashing it. Hashing is a process of converting data into a fixed-size string of characters that cannot be reversed to obtain the original data. The use of salting makes the resulting hash more difficult for attackers to crack using brute force attacks.
\subsubsection{Tenant's Detection module (Local Detection):} Each tenant assumes the responsibility of training a model to detect malicious behavior among its users and subsequently monitoring them based on this model. This approach not only ensures the security of each tenant's data associated with their users but also allows for customization based on the individual preferences of each tenant. By conducting this section and monitoring within each tenant's environment, a higher level of control and flexibility can be achieved, enabling tailored security measures to be implemented according to the specific needs and preferences of each tenant.
\subsubsection{Tenant's Adaptation module (Local Adaptation):} It contains two sub modules:
\begin{itemize}
   \item \textbf{Adaptation Decision Engine:} This Module estimates the cost of possible adaptation actions and selects the ones that have the lowest cost for the system.  It takes into account the dependencies between the tasks in the workflow and identifies which other tasks should be adapted in addition to the violated task to prevent the propagation of already occurred violations. For instance, if a task is skipped, the Adaptation Decision Engine ensures that the subsequent tasks that depend on the skipped task are also adapted accordingly.
   \item \textbf{Tenant-level Adaptation:} This module is responsible for adapting the violated and potentially violated tasks in the already running instances. It takes appropriate actions such as skipping a task, re-sequencing the process, or inserting a new task to compensate for the effect of the occurred violations. These actions are at the process level and are designed to fully or partially mitigate the impact of the violations on the overall workflow.
 \end{itemize}
 
\subsection{Navigator}
This module is crucial for ensuring the efficient management and scheduling of tasks for all tenants' kernels in the cloud environment. It plays a vital role in ensuring the overall behavior of the cloud environment by continuously monitoring the resources and services available and matching them with the requirements of the submitted tasks. Additionally, the module can detect and adapt the security violations in the cloud environment to ensure that tenants continue to receive the best possible performance from the cloud services.
  
\subsubsection{Trust-aware Scheduling planner} The main function of this module is to schedule the workflow and allocate suitable cloud services for each task based on each tenant's specific requirements, such as cost, time, and security. The module seeks to balance conflicting needs and ensure that the demands of tenants are met. In addition, the module takes into account security constraints by considering the separation patterns generated in the previous stage, as well as the trustworthiness of providers. The trustworthiness of providers is regularly updated through the Provider Trust Adaptation module, which maintains a repository of provider trust information used by the scheduler. In addition, this module is responsible for anonymizing the tenants' specifications in the tasks before they are sent to the cloud for execution. This is similar to the Task Anonymizer module which is located on the tenant side.

\subsubsection{Global Monitoring and Detection}
\label{Section:Global Detection}
This module is responsible for real-time monitoring of the cloud behavior by analyzing the cloud log file and the network traffic data. It includes two main modules discussed below:
  \begin{itemize}
  \item \textbf{Service Training Model:} 
The main purpose of this module is to train a robust machine learning model that can detect any malicious behavior in the cloud by analyzing the real-time network traffic data and cloud log files. The model is trained using various parameters such as protocol type,  duration, and number of packets from the network traffic data sets. Additionally, the cloud log file is also analyzed to extract information on CPU utilization, bandwidth consumption, and RAM utilization. By analyzing these parameters, the model can identify any anomalies or abnormal patterns in the cloud behavior that may indicate a potential security breach or attack.
\item \textbf{Service monitoring:} The Service Monitoring module uses the machine learning model created by the Provider Training module to detect any malicious activity in the cloud services and providers. It continuously analyzes the real-time network traffic data and cloud log file, comparing them with the expected behavior derived from the trained model. In case of any anomalies or suspicious activity, the module immediately raises an alert to the adaptation module, which will take the necessary measures to mitigate the risk and ensure the overall security of the cloud environment. 
 \item \textbf{Rule-based Tenant’ IDS:} 
  \item \textbf{Rule-based Tenant’ IDS:}  It involves a set of predefined rules to identify potential attacks from tenants. These rules can be based on various factors, such as the number of detected malicious users during the specific period, The number of active users during the specific period, Max/Min duration of a user task. Based on these rules, we can detect malicious tenants during a specific period of time and take appropriate action to investigate and respond to them.
 \end{itemize}
 

\subsubsection{Global Adaptation}
\label{Global Adaptation}
The Global Adaptation module is critical for ensuring efficient adaptation in the level of services and providers in response to the detected violations or security threats. it comprises two modules that are described in detail below:
   \begin{itemize}
   
    \item \textbf{Middle-ware level Adaptation:} This module enables the adaptation of services by taking appropriate actions at the middle-ware level. These actions may include changing the services within the same provider or selecting a service from another provider that meets the tenant's requirements. By doing so, the module ensures the fulfillment of the tenant's needs and maintains the required level of service quality.
   \item \textbf{Provider Trust Adaptation:} It updates the trust level of the providers based on any detected violations or security threats. The trust repository of the providers and services is updated accordingly, which improves the scheduling decisions for future workflow instances. These updated trust values are utilized by the Trust-aware scheduling planner to schedule upcoming workflow instances, thus enhancing the overall security and efficiency of the system. Additionally, this module may modify the Provider Prediction model to improve the monitoring of malicious provider behavior with greater precision.
 \item \textbf{Tenant Trust Adaptation:} It will update the tenants' trust level and based on it, the proper adaptation action will be taken (e.g. monitoring the behavior of the tenant with more precision (shown as \textbf{b2}), restricting the tenant's access, blocking the tenant's activities, or even ignoring the alert if the updated trust is upper than the defined threshold).
    \item \textbf{Resource Violation Propagation Analysis:} This component takes the alert from the Provider Prediction model and then, Based on created Resource Violation Propagation Patterns, it will decide if this violation will be propagated to the other workflow instances or not. As an example, if an attack (such as a DOS attack) occurs in one cloud service, the other workflow instances that intend to use this service may also be affected by the attack. After identifying the potential violated tasks in the workflow instances, it will send an alert to notify the corresponding tenants to do proper adaptations
 \end{itemize}
 


 

==> Sections/System_Model.tex <==
 \section{ Problem description and Motivation Scenario}
The security and privacy of workflows executed in a multi-cloud environment are crucial concerns for businesses and organizations. In such an environment, several security and privacy violations may occur, such as unauthorized access to sensitive data, data leakage, unauthorized modification, and unavailability of cloud services and results. These violations can cause significant damage to the workflow execution and the overall system's security, making it necessary to address them. Therefore, the main problem we aim to address in this paper is all of these violations that may occur during the execution of workflows in a multi-cloud environment. Our main focus is to identify such risks and violations and propose measures to adapt them. To tackle this problem, in this section, we will describe the different modules in our system model and identify potential adversaries that may pose a threat to the system's security.

\textbf{Tenants:} As our system operates in a multi-tenant environment, each tenant must be able to model, execute, monitor, and adapt their workflows based on their security requirements and strategies in an isolated environment provided by the engine.

\textbf{WfMS (Workflow Engine):} The Workflow Engine is responsible for managing tenant workflow execution in a secure and efficient manner. It must ensure that tenants can use cloud services securely and assist them in detecting and adapting to potential attacks.

\textbf{Multi-Cloud Environment:} A Multi-Cloud Environment is a set of multiple cloud providers, each of which provides different offers. Each Cloud Provider is an entity that can provide multiple cloud offers as different services.

Figure \ref{Figure_systemModel} illustrates our system model.

\begin{figure}[bth!]
\includegraphics[width=\columnwidth]{figures/system model.pdf}
\caption{System Model}
\label{Figure_systemModel}
\end{figure}

\subsection{Adversary Model}

Our adversary model considers the possibility of malicious behavior from various entities involved in the system, including cloud users, engine users (tenants), providers (such as a dishonest provider administrator or high-privileged malicious cloud software), or even the engine itself.

\subsubsection{The Engine}
We assume that the engine is semi-trusted and susceptible to attacks. In a multi-tenant environment, the engine will attempt to learn as much as it can about tenants and their sensitive data. However, the engine does not have access to the isolation environments provided for each tenant.

\subsubsection{The Engine Users (Tenants)}
In a multi-tenant environment, engine users (tenants) can be potential attackers. Malicious tenants can bypass the isolation environments provided for each tenant and attack other tenants' assets to gain access to their sensitive information or manipulate their tasks and data.

\subsubsection{The Providers}
We assume that the cloud is semi-trusted and susceptible to attacks. Therefore, cloud services (e.g. a client at the cloud service provider side) and resources are not fully trusted, and their behavior should be monitored. Additionally, a malicious cloud provider (e.g. a dishonest provider administrator, high-privileged malicious cloud software, etc.) can be a potential attacker, as it can infer sensitive information by combining the knowledge of workflow logic.

\subsubsection{External Attackers}
The shared nature of cloud infrastructure, where computing and storage resources are shared with other users, can also be a source of attacks. An external attacker, which can be a malicious cloud user or other external users (e.g. a network attacker outside the cloud network), carries out attacks through the Internet and disrupts the services provided to legitimate users \cite{Modi2017}. In our case, they can attack tenant assets when they are being executed in the providers.

The goal of attacks from potential attackers in our scenario is to gain unauthorized access to private assets or modify workflow assets.

\subsection{Motivation Scenario}
In this section, we present an illustrative example to highlight potential security risks that may arise during the execution of workflows in a multi-cloud environment. Our case study is based on the insurance claim recovery chain \cite{Goettelmann2015a}, which is depicted in the accompanying BPMN diagram and comprises several tasks  \ref{figure_bpmnExample}. This workflow is initiated by a customer who submits a claim recovery declaration to the tenant (the customer's insurance company), which owns the workflow. The declaration contains sensitive information, such as the customer's name, address, and bank account details.

Upon receiving the claim recovery declaration, the emergency service is immediately notified to obtain incident details. Subsequently, three parallel tasks are executed, including requesting claim documents, hospital reports, and police reports, based on the incident details. An expert then decides on reimbursement, and then two parallel tasks will be executed which are notifying the customer about the reimbursement Decision and requesting the bank if it is the case(the reimbursement Decision is positive).

To ensure the security of this workflow, it is imperative to protect the customer's private information, particularly during the transmission and processing of data across multiple insurance companies and cloud environments. Furthermore, it is vital to maintain the confidentiality of the process logic for sensitive tasks, such as obtaining an expert report, to prevent unauthorized access. Overall, this example emphasizes the significance of robust security measures in multi-cloud environments to ensure the protection of sensitive data and mitigate potential security breaches.
\begin{figure*}[h]
  \includegraphics[width=\textwidth]{figures/diagram_1.png}
  \caption{}
  \label{figure_bpmnExample}
\end{figure*}

==> Sections/draft-Evaluation.tex <==
 \section{Evaluation}
 In this section, we want to evaluate the effectiveness of the proposed solution. To achieve this, we have successfully implemented SecFlow by extending the jBPM (Java Business Process Management) engine and integrating it with the cloudPlus simulation tool. jBPM, known for its lightweight and fully open-source nature, offers a pluggable architecture that allows for seamless removal of coupling and easy replacement of different implementations. Additionally, the integration of the comprehensive simulation framework, Cloudsim Plus, has empowered us to accurately model the complexities of a multi-cloud environment. we conducted experiments in a simulated environment using the following setup.
 \subsection{Example Scenario}
 Figure \ref{} shows a BPMN example along with the required specification. Our case study revolves around the insurance claim recovery chain \cite{Goettelmann2015a}, which we have depicted using a BPMN diagram (see Figure \ref{figure_bpmnExample}). This workflow consists of several tasks, each contributing to the overall claim recovery process. It is important to note that the information shared within this workflow is sensitive, encompassing details such as the customer's name, address, and bank account information. The workflow begins when a customer submits a claim recovery declaration to the tenant, which is their insurance company and the owner of the workflow. Upon receipt of the claim recovery declaration, the incident details service is promptly notified to retrieve relevant incident information. Subsequently, three parallel tasks are executed: requesting claim documents, hospital reports, and police reports, based on the obtained incident details. An expert then makes a decision regarding the reimbursement, which triggers the Band Reimbursement service if the claim is accepted. The customer is subsequently notified of the reimbursement decision. Finally, the customer is invited to provide feedback about the company and the overall process.To address the security concerns associated with this example, we have defined specific security requirements for each task. These requirements encompass aspects such as integrity, confidentiality, and availability of the information involved. Furthermore, we have outlined feasible adaptation actions that can be implemented at both the tenant and middleware levels to mitigate potential security risks and ensure compliance with the defined security requirements.
 
\subsection{Experimental Setting }
 In this section, we described our settings for different parts of the experiments. For the learning phase in the service training module, we create the required dataset including the network traffic data and cloud logfile for the motivation workflow scenario by simulating different types of attacks in services and networks. In this paper, we specifically focused on four prevalent types of attacks in cloud services and networks including Denial of Service (DoS), Remote-to-Local (R2L), User-to-Root (U2R), and probe attacks. Then we train the attack detection model and also the attack severity model using these logfiles. Then we use this model to have real-time monitoring data and detect security violations. 

\subsection{main results}
We evaluated the proposed solution using multiple workflow models, each consisting of different numbers of service tasks and exhibiting various control and data dependencies. Our evaluation focused on the following key aspects:

Attack Detection: We measured the accuracy and efficiency of the attack detection module in identifying security violations during workflow execution. This evaluation provided insights into the system's ability to detect attacks in real-time and mitigate their impact.

Adaptation Effectiveness: We assessed the effectiveness of the adaptation module in selecting and executing appropriate adaptation actions to mitigate the impact of detected attacks. This evaluation considered factors such as the reduction in attack severity, resource utilization, and workflow performance.

Scalability: We examined the scalability of the proposed solution by varying the size and complexity of the workflow models. This evaluation aimed to determine the system's performance and resource requirements as the workload and number of tasks increased.

Comparative Analysis: We compared the performance of the proposed solution against existing methods or alternative approaches in terms of attack detection accuracy, adaptation effectiveness, and overall system performance. This analysis provided insights into the advantages and limitations of our solution compared to other techniques.

We present the detailed experimental results and analysis in the following section.



\begin{align}
X_{normalized\underset{X \in \{P, T, MS, V\}}{(aa)}} = \begin{cases}
X_{aa} & \text{if } |finalAA| = 1 \\
0 & \text{if } |finalAA| > 1 \text{ and } maxX = minX \\
\frac{X_{aa} - minX}{maxX - minX} & \text{if } |finalAA| > 1 \text{ and } maxX \neq minX \\
\end{cases}
\label{eq:Normalized}
\end{align}


In Equation \ref{eq:Normalized}, X can represent the price, time, or value for a specific adaptation action $aa$. The variables $maxX$ and $minX$ correspond to the maximum and minimum values among the adaptation options for the respective X. The formula considers three scenarios: a)If there is only one adaptation action ($|finalAA| = 1$), no normalization is needed, and the original value, denoted as $AX_{aa}$, is used. b) If there are multiple adaptation actions and the maximum and minimum values are the same ($maxX = minX$), indicating equal values for all options, the normalized value is set to 0. c) For multiple adaptation actions with different maximum and minimum values ($maxX \neq minX$), the normalized value is calculated as $\frac{AX_{aa} - minX}{maxX - minX}$.

The given formula represents the process of calculating the normalized values for the price, time, and value of different adaptation actions. This calculation is performed in Equation \ref{eq:Normalized}, which builds upon the concepts introduced in Equation \ref{eq:AdaptationCost}.

In Equation \ref{eq:Normalized}, the variable $AX_{normalized\underset{X \in {P, T, V}}{(aa)}}$ represents the normalized value of a specific factor (price, time, or value) for an adaptation action $aa$. The subscript $X \in {P, T, V}$ indicates that $X$ can take on values from the set ${P, T, V}$, which corresponds to the factors of price, time, and value.

The formula within the cases environment specifies three different cases for calculating the normalized value, depending on the conditions:

If there is only one adaptation action available for the detected attack, indicated by $|finalAA| = 1$, there is no need for normalization. In this case, the normalized value remains the same as the original value ($AX_{aa}$).

If there are multiple adaptation actions ($|finalAA| > 1$) and the maximum and minimum values of the factor are equal ($maxX = minX$), it implies that all adaptation options have the same value for that factor. In such cases, the normalized value is set to 0.

If there are multiple adaptation actions ($|finalAA| > 1$) and the maximum and minimum values of the factor are different ($maxX \neq minX$), the normalized value is calculated by subtracting the minimum value ($minX$) from the original value ($AX_{aa}$) and dividing the result by the range of values ($maxX - minX$). This normalization process scales the values between 0 and 1.

The explanation further clarifies that in Equation \ref{eq:Normalized}, the variable $X$ can represent the price, time, or value for the adaptation action $aa$. The variables $maxX$ and $minX$ correspond to the maximum and minimum amounts for the respective factor (price, time, or value). The conditions $|finalAA| = 1$ and $maxX = minX$ are used to handle specific scenarios and ensure appropriate normalization when necessary.

==> Sections/draft.tex <==
\begin{align}
 AdaptedPrice(aa, t_i) =\frac{{AdaptationActionPrice(aa, t_i) - NormaPrice}(t_i)}{{NormaPrice(t_i)}}
 \label{Equation:AdaptedPrice}
\end{align}
Equation \ref{Equation:AdaptedPrice} calculates the cost of adaptation action $aa$ based on the type of adaptation.

\begin{align}
AdaptedTime(aa, t_i) = \frac{{AdaptationActionTime(aa, t_i) - NormalTime(t_i)}}{{NormalTime(t_i)}} 
\label{Equation:AdaptedTime}
\end{align}

\begin{align}
 RiskMitigation(aa, t_i) =\frac{{SecurityRisk(aa,t_i) -AttackScore(a_k, t_i, s_j)}}{{AttackScore(a_k, t_i, s_j)}} 
 \label{Equation:RiskMitigation}
\end{align}

\begin{align}
\text{AdaptedValue}(aa, t_i) &= \frac{{\text{Value}(w, aa) - \text{Value}(w)}}{{\text{Value}(w)}}
\label{Equation:AdaptedValue}
\end{align}

\noindent $AdaptationCost(aa, t_i) =$
\begin{align}
\begin{split}
 &\quad \noindent AdaptationCost(aa) = W_{price} \cdot AP_{normalized}(aa) + \\
&\quad W_{time} \cdot AT_{normalized}(aa) -  W_{value} \cdot AV_{normalized}(aa)
\end{split}
\label{Equation:AdaptationCost}
\end{align}




\subsection{Adaptations}
The responsible module for applying each adaptation action will be defined. We have two modules which are responsible for applying the adaptation actions. The first one is The middleware adaptation module is a crucial component for handling adaptations resulting from changes in providers and cloud services. Its main objective is to simplify middle-level adaptations, easing the burden on tenants. Specifically, it focuses on re-configuration and task re-execution requirements in the adaptation process.
 Configuration adaptation involves adjusting the settings of specific cloud services to improve future decision-making in different modules. This includes modifying the trust level of cloud services within the scheduling module and changing the Attack Frequency Rate (AFR) used in the Adaptation Decision Engine for calculating the attack score.


\subsubsection{Tenant-level Adaptation}
In this section, we want to perform the tenant-level adaptation which comprises the skip and re-sequencing of the tasks. The tenant is responsible for applying the adaptation actions which is related to the business process level. based on the selected


\subsubsection{Middle-ware level Adaptation}
The middleware adaptation module is a crucial component for handling adaptations resulting from changes in providers and cloud services. Its main objective is to simplify middle-level adaptations, easing the burden on tenants. Specifically, it focuses on re-configuration and task re-execution requirements in the adaptation process.

In addition to configuration adaptation, the middleware adaptation module provides the option of re-executing tasks in the case that any violation is detected. This allows the navigator to respond to security violations by rerunning affected tasks with modifications or alternative approaches to ensure workflow security. Two options are available for task re-execution. 

The first option is to continue running the task with the same cloud provider while implementing additional security measures. This involves using a different Service Level Agreement (SLA) that provides enhanced security guarantees. The navigator can negotiate with the cloud provider to enforce stricter security controls, particularly for data transfer. This option is suitable when the violation is detected in network traffic data, indicating no malicious behavior within the cloud services.

The second option is to rerun the task using a different cloud provider. In this case, the navigator switches to a different cloud provider to achieve a higher level of security and reduce the likelihood of future security violations. This option is chosen when the violation is detected in the cloud log file, indicating malicious cloud behavior or an ongoing attack.



\subsection{Provider Trust Adaptation}

 \input{Algorithms/Periodic Trust Update Algorithm for Providers}









It begins by splitting the network traffic dataset into training and testing sets. It then proceeds to train a Random Forest model on the training data by building an ensemble of decision trees. Once the Random Forest model is trained, its performance is evaluated on the testing data. The model is applied to the testing dataset, and the accuracy is calculated to determine how well it predicts the presence or absence of attacks. 


\label{Tenant’s Kernel}
 The Tenant's Kernel provides an isolated environment for each tenant where they can model, analyze and adapt workflows based on their requirements and strategies. This ensures that the decisions and data of one tenant are protected from other tenants. It consists of the following four sub-modules. 1)\textit{Workflow Modeller}
\label{Section:Security Modeller}
The Workflow Modeller module enables tenants to model their workflows in a secure and efficient way. During the modeling process, the security requirements (confidentiality, integrity, and availability) of each task are defined. 

\subsubsection{Security Evaluator}
\label{Section:Security Evaluator}
 In this module, the possible adaptation actions for each task are defined here. This requires establishing a set of adaptation strategies (e.g., skipping, re-working, re-sequencing, re-configuration) for each task in the workflow model and determining their potential impact on the overall value of the workflow and on the balance between value and security properties. As an example of such specification, consider the scenario of skipping certain tasks within the workflow, some tasks may be less critical, and skipping them may have little impact on the overall workflow value. However, for other tasks, such as authentication tasks, skipping is not even an option in case of any violation, as they are essential to the security of the workflow. In such cases, the impact of skipping could be significant and compromise the overall security of the workflow. Therefore, by incorporating such specifications for each task in the security evaluator module after the modeling phase, the cost of each adaptation action could be estimated in execution time, thus allowing to select the most viable adaptation option for any violations that may arise. 

\subsubsection{Task Anonymizer }
\label{Section:Task Anonymizer}
This module is responsible for handling sensitive input data in a secure and efficient manner in a cloud computing environment. To achieve this, it utilizes appropriate obfuscation techniques to anonymize sensitive information before submitting tasks to the navigator for scheduling and allocation to the planned cloud services and resources for execution. This sensitive information for each task includes all unnecessary information for processing that task such as Workflow-ID, Instance-ID, names, addresses, etc. After execution, this obfuscated information is included in the intermediate results for upcoming tasks, if needed. It utilizes appropriate obfuscation techniques such as tokenization and salting to ensure the security of sensitive data. Tokenization involves replacing sensitive data with a unique identifier or token, while salting involves adding a random string of characters to the sensitive data before hashing it. Hashing is a process of converting data into a fixed-size string of characters that cannot be reversed to obtain the original data. The use of salting makes the resulting hash more difficult for attackers to crack using brute force attacks.
\subsubsection{Tenant's Detection module (Local Detection):} Each tenant assumes the responsibility of training a model to detect malicious behavior among its users and subsequently monitoring them based on this model. This approach not only ensures the security of each tenant's data associated with their users but also allows for customization based on the individual preferences of each tenant. By conducting this section and monitoring within each tenant's environment, a higher level of control and flexibility can be achieved, enabling tailored security measures to be implemented according to the specific needs and preferences of each tenant.
\subsubsection{Tenant's Adaptation module (Local Adaptation):} It contains two sub modules:
\begin{itemize}
   \item \textbf{Adaptation Decision Engine:} This Module estimates the cost of possible adaptation actions and selects the ones that have the lowest cost for the system.  It takes into account the dependencies between the tasks in the workflow and identifies which other tasks should be adapted in addition to the violated task to prevent the propagation of already occurred violations. For instance, if a task is skipped, the Adaptation Decision Engine ensures that the subsequent tasks that depend on the skipped task are also adapted accordingly.
   \item \textbf{Tenant-level Adaptation:} This module is responsible for adapting the violated and potentially violated tasks in the already running instances. It takes appropriate actions such as skipping a task, re-sequencing the process, or inserting a new task to compensate for the effect of the occurred violations. These actions are at the process level and are designed to fully or partially mitigate the impact of the violations on the overall workflow.
 \end{itemize}
 
\subsection{Navigator}
This module is crucial for ensuring the efficient management and scheduling of tasks for all tenants' kernels in the cloud environment. It plays a vital role in ensuring the overall behavior of the cloud environment by continuously monitoring the resources and services available and matching them with the requirements of the submitted tasks. Additionally, the module can detect and adapt the security violations in the cloud environment to ensure that tenants continue to receive the best possible performance from the cloud services.
  
\subsubsection{Trust-aware Scheduling planner} The main function of this module is to schedule the workflow and allocate suitable cloud services for each task based on each tenant's specific requirements, such as cost, time, and security. The module seeks to balance conflicting needs and ensure that the demands of tenants are met. In addition, the module takes into account security constraints by considering the separation patterns generated in the previous stage, as well as the trustworthiness of providers. The trustworthiness of providers is regularly updated through the Provider Trust Adaptation module, which maintains a repository of provider trust information used by the scheduler. In addition, this module is responsible for anonymizing the tenants' specifications in the tasks before they are sent to the cloud for execution. This is similar to the Task Anonymizer module which is located on the tenant side.

\subsubsection{Global Monitoring and Detection}
\label{Section:Global Detection}
This module is responsible for real-time monitoring of the cloud behavior by analyzing the cloud log file and the network traffic data. It includes two main modules discussed below:
  \begin{itemize}
  \item \textbf{Service Training Model:} 
The main purpose of this module is to train a robust machine learning model that can detect any malicious behavior in the cloud by analyzing the real-time network traffic data and cloud log files. The model is trained using various parameters such as protocol type,  duration, and number of packets from the network traffic data sets. Additionally, the cloud log file is also analyzed to extract information on CPU utilization, bandwidth consumption, and RAM utilization. By analyzing these parameters, the model can identify any anomalies or abnormal patterns in the cloud behavior that may indicate a potential security breach or attack.
\item \textbf{Service monitoring:} The Service Monitoring module uses the machine learning model created by the Provider Training module to detect any malicious activity in the cloud services and providers. It continuously analyzes the real-time network traffic data and cloud log file, comparing them with the expected behavior derived from the trained model. In case of any anomalies or suspicious activity, the module immediately raises an alert to the adaptation module, which will take the necessary measures to mitigate the risk and ensure the overall security of the cloud environment. 
\item \textbf{Rule-based Tenant’ IDS:}  It involves a set of predefined rules to identify potential attacks from tenants. These rules can be based on various factors, such as the number of detected malicious users during the specific period, The number of active users during the specific period, Max/Min duration of a user task. Based on these rules, we can detect malicious tenants during a specific period of time and take appropriate action to investigate and respond to them.
 \end{itemize}
\subsubsection{Global Adaptation}
\label{Global Adaptation}
The Global Adaptation module is critical for ensuring efficient adaptation in the level of services and providers in response to the detected violations or security threats. it comprises two modules that are described in detail below:
   \begin{itemize}
 
  \item \textbf{Service Adaptation:} This module enables the adaptation of services by taking appropriate actions at the middle-ware level. These actions may include changing the services within the same provider or selecting a service from another provider that meets the tenant's requirements. By doing so, the module ensures the fulfillment of the tenant's needs and maintains the required level of service quality.
    
 \item \textbf{Tenant Trust Adaptation:} It will update the tenants' trust level and based on it, the proper adaptation action will be taken (e.g. monitoring the behavior of the tenant with more precision (shown as \textbf{b2}), restricting the tenant's access, blocking the tenant's activities, or even ignoring the alert if the updated trust is upper than the defined threshold).
 
   \item \textbf{Provider Trust Adaptation:} It updates the trust level of the providers based on any detected violations or security threats. The trust repository of the providers and services is updated accordingly, which improves the scheduling decisions for future workflow instances. These updated trust values are utilized by the Trust-aware scheduling planner to schedule upcoming workflow instances, thus enhancing the overall security and efficiency of the system. Additionally, this module may modify the Provider Prediction model to improve the monitoring of malicious provider behavior with greater precision.

    \item \textbf{Resource Violation Propagation Analysis:} This component takes the alert from the Provider Prediction model and then, Based on created Resource Violation Propagation Patterns, it will decide if this violation will be propagated to the other workflow instances or not. As an example, if an attack (such as a DOS attack) occurs in one cloud service, the other workflow instances that intend to use this service may also be affected by the attack. After identifying the potential violated tasks in the workflow instances, it will send an alert to notify the corresponding tenants to do proper adaptations
 \end{itemize}
 


 


\textbf{Definition 1 (Task)}: A task $t$ represents a service task that utilizes a cloud service for execution. It is defined as a tuple ($C_t$, $I_t$, $A_t$, $AA_t$), where $C_t$, $I_t$, and $A_t$ represent the Confidentiality, Integrity, and Availability requirements of the task $t$, respectively. Additionally, $AA_t$ indicates the feasible adaptation actions that can be performed on task $t$ in response to any violations.

\textbf{Definition 2 (Workflow)}: A Workflow, $W$, is a tuple (T, D, $E_c$, $E_d$) where T is a set of tasks $t \in T$, D is the set of data, $E_c$ is a set of control edges that define the order in which the tasks are performed based on the set of conditions that must be met  $E_c \subset T\times T\times Conds(D)$, $E_d$ is a set of data edges that specify the flow of data between the tasks $E_d \subset T\times T\times D$.

\textbf{Definition 3 (Attack)}: An attack $a$ is a security violation that may occur during the execution of a workflow $W$ in task $t$, compromising the security of task $t$. It is defined as a tuple ($C_a$, $I_a$, $A_a$, $AA_{a_H}$,$AA_{a_M}$,$AA_{a_L}$), where $C_a$, $I_a$, and $A_a$ represent the impacts of the attack $a$ on confidentiality, integrity, and availability, respectively. Additionally,  $AA_{a_H}$, $AA_{a_M}$, and $AA_{a_L}$ represent the adaptation actions that can be taken to mitigate the impact of attack $a$ with different severity levels, namely High, Medium, and Low, respectively.

\textbf{Definition 3 (Service)}: A service $s$ represents a service in the provider $p$. it is defined as a tuple ($C_s$, $I_s$, $A_s$, $AFR$) in which $C_s$, $I_s$, $A_s$ are Confidentiality, Integrity, and Availability that this service provides respectively, and AFR is the attack frequency rate of service $s$ for different types of attacks. $AFR = \bigcup_{A \in \text{AttackTypes}} AFR_A$






\textbf{Definition 2 (Multi-Cloud Environment)} A Multi-Cloud Environment, CPs, is a set of multiple cloud providers each of which provides different offers: \begin{equation}  CPs = \{ CP_i | 0 \leq i < m, m=|CPs| \} \end{equation}

\textbf{Definition 3 (Cloud Provider)} A Cloud Provider, $CP_i$, is an entity which can provide multiple cloud offers. It is defined as $CP_i$ = ⟨$id_i$, $Rs_i$⟩, where:
\begin{enumerate}
  \item 	$id_i$ is the unique identifier of $CP_i$;
  \item 	$Rs_i$  is a set of cloud resources provided by $CP_i$  so that:
\begin{equation} Rs_i=\{R_{i_k} |0 \leq i < m, 0 \leq k < r, r=|Rs_i|\}\end{equation}
\end{enumerate}

\textbf{Definition 4 (Workflow engine)} The Workflow Engine is responsible for executing the workflows in a secure and efficient manner. It enables users to define and model workflows and supports the enactment, management, and analysis of operational processes. To execute the workflows, the Workflow Engine first creates a Cloud Service Composition plan and then selects the appropriate cloud service to execute each task. The Cloud Service Composition is defined as follows:

\textbf{Definition 4 (Cloud Service Composition)} A cloud service composition
is defined as CSC = ⟨SCP, SCSs⟩, where:
\begin{enumerate}
 \item SCP is the corresponding cloud service composition plan;
 \item SCSs is the set of cloud services selected for tasks T , where
for each task $t_j$ in T , there is one CS in SCSs to fulfill $t_j$.
\begin{equation} SCSs=\{\forall t_j \in T (\exists CS \in SCSs | \,CS \, executes\, t_j)\}\end{equation}
\end{enumerate}


1) Rerun the task with the same cloud provider without any migration. This adaptation will be adopted when the occurred violation is detected in the network traffic data which means that there is no malicious behavior inside the cloud services.

Option 1: Continue running the task with the same cloud provider while implementing additional security measures to minimize the risk of a similar security violation occurring. This option involves running the task with a different Service Level Agreement (SLA) that provides enhanced security guarantees. The navigator may negotiate with the cloud provider to enforce stricter security controls to protect the transferring of data. This adaptation will be adopted when the occurred violation is detected in the network traffic data which means that there is no malicious behavior inside the cloud services.

Option 2: Rerun the task by using a different cloud provider. In this scenario, the navigator decides to switch to a different cloud provider to ensure a higher level of security and reduce the likelihood of future security violations. The task is migrated to the new cloud provider, and appropriate adaptations are made to ensure compatibility and integrity during the migration process. This option provides an opportunity to leverage the security capabilities of a different cloud provider and benefit from their specialized security measures and infrastructure.



\textit{Adapted Price:} This is the normalized price that the selected adaptation action will contribute to the overall execution cost of the workflow.

\begin{align}
 AdaptedPrice(AA, t_i) =\frac{{AdaptationActionPrice(AA, t_i) - NormaPrice}(t_i)}{{NormaPrice(t_i)}}
 \label{Equation:AdaptedPrice}
\end{align}


\textit{Adapted Time:} This is the normalized time that the selected adaptation action will add to the overall execution time of the workflow.

\begin{align}
AdaptedTime(AA, t_i) = \frac{{AdaptationActionTime(AA, t_i) - NormalTime(t_i)}}{{NormalTime(t_i)}} 
\label{Equation:AdaptedTime}
\end{align}

\textit{Risk Mitigation Factor:} It is the normalized Risk Mitigation Factor that the selected adaptation action will provide to the whole security of the execution of the workflow. It is calculated by considering the security risk of the adaptation action and Then normalizing it using the attack score.

\begin{align}
 RiskMitigation(AA, t_i) =\frac{{SecurityRisk(AA,t_i) -AttackScore(A, t_i, s_j)}}{{AttackScore(A, t_i, s_j)}} 
 \label{Equation:RiskMitigation}
\end{align}

\textit{Adapted Value:} It is the normalized value that the selected adaptation action will provide to the whole workflow and Then normalizing it using the attack score.

\begin{align}
\text{AdaptedValue}(AA, t_i) &= \frac{{\text{Value}(w, AA) - \text{Value}(w)}}{{\text{Value}(w)}}
\label{Equation:AdaptedValue}
\end{align}






\subsection{Separation pattern}

Each tenant in the \textit{Security Evaluator} module (section \ref{Section:Security Evaluator}), will define a set of the Confidentiality Requirements for each workflow as \textit{separation patterns} along with workflow model. These patterns preserve data and logic privacy for different entities including instances, users, and tenants.

Definition 1 (Instance Separation Pattern). This separation pattern shows the confidentiality relationship between tasks in one instance. In other words, it expresses if one cloud has two or more tasks of one instance, it can infer additional privacy information by combining multiple pieces of such data. This pattern is represented as a t*t-dimensional matrix (t = |Tasks |), where 〖SP〗_instance[i][j]=1 (i,j∈Tasks) indicates whether  t_i   and t_j shouldn’t assign to same cloud provider.
〖SP〗_instance [i][j]={█(1       t_i  ,t_j  shouldn’t assign to the same cloud @0                           no restriction between t_i,t_j  )┤

Example 1. The follow example shows the propagation pattern of the motivation scenario. As the ”initiate claim” task includes the private data from the customer (like name, address, bank account info, and etc.), the customer’s identity should be anonymized in the task’s output data, otherwise the confidentiality degree of this data will be propagate to the all following tasks. This matrix indicates that t_0 shouldn’t be located at the same cloud with the other tasks as all of the referred values are 1. Also, as there is no other restriction for the further tasks, the other values are 0.
                                    ■(t_0&t_1&t_2&t_3&t_4&t_5&t_6 )
P_Propagation=■(t_0@t_1@t_2@t_3@t_4@t_5@t_6 ) [■(0&1&1&1&1&1&1@1&0&0&0&0&0&0@1&0&0&0&0&0&0@1&0&0&0&0&0&0@1&0&0&0&0&0&0@1&0&0&0&0&0&0@1&0&0&0&0&0&0) ]


Definition 2 (User Separation Pattern). This pattern preserves the confidentiality of the users involved in the workflow by preventing a single cloud from executing all critical tasks related to a user. This pattern is represented as a t*u-dimensional matrix (u = |Users |) , where 〖SP〗_user[i][j]=v (i∈Tasks,j∈Users) indicates the maximum number of t_i tasks from different instances belonging to the u_j that can be assigned to one cloud provider. 

                                   


Example 2. In the motivation scenario, there are four users involved in the instances: Client, Police, Hospital, and Expert. As an example, if one cloud has all instances related to the one client, it can infer number of her/his accident, history of her/his medical treatment, etc. So, based on the separation rate, we can define the maximum number of allowed instances of each user assigned to one cloud in the specific time  period.
                         ■(t_0   &t_1& t_2& t_3&〖 t〗_4& t_5& t_6 )
〖SP〗_user=■(u_0@u_1@u_2@u_3 ) [■(3&0&0&0&0&0&3@0&0&10&0&0&0&0@0&0&0&20&0&0&0@0&0&0&0&5&0&0) ]

Definition 3 (Tenant Separation Pattern). This pattern try to preserve the data and logic privacy of each tenant by preventing a single cloud from executing all critical tasks related to a tenant. This pattern is represented as a t-dimensional matrix, where 〖SP〗_tenant [i]=1 (i∈Tasks) indicates that the set of t_i   tasks from different instances belonging to one tenant shouldn’t assign to one cloud provider. Also, r_seperation is a m-dimensional matrix (m = |Tenants |)  where r_seperation [k]=v (k∈Tenants) and v shows the maximum number of tasks from different instances belonging to tenant k that can be assigned to one cloud provider.

                                   


Example 2. In the motivation scenario, if one cloud has all instances related to one tenant (insurance company), it can infer the information like the number of its clients and their specifications, the total amounts and taxes, etc. So, based on the separation rate, we can define the maximum number of allowed instances of each tenant assigned to one cloud in the specific time period.
                                ■(t_0&t_1&t_2&t_3&t_4&t_5&t_6 )
                                                〖SP〗_tenant= [■(1&0&0&0&0&0&1) ]

                                 ■(〖tenant〗_(0  )  &〖tenant〗_(1 )  &〖tenant〗_2 )
 		 		r_seperation= [■(10       &12           &6) ]







==> Sections/draftRL.tex <==
\item \textbf{State}: Represents the set of all possible states. Each state is defined by a 3-tuple $st=(St_T, St_W, St_P)$, where $St_T$ denotes the current state of the task and any detected violations, $St_W$ signifies the present state of the workflow, and $St_P$ describes the existing state of the various services provided by all providers in relation to their workload.


These uncertain overhead costs such as when the provider load exceeds a predefined threshold, the "Rework" action on that particular provider may result in additional costs. Similarly, if the "insert" action is applied and other tasks within the workflow have already been replaced due to prior violations, it may lead to uncertain overhead costs. Additionally, the "skip" action in certain tasks can give rise to randomly unhandled overhead, thereby increasing both the time and cost implications throughout the workflow. These conditions underscore the complexities involved in selecting the most suitable adaptation action and evaluating its overall performance.

==> Sections/draft_architecture.tex <==
\subsubsection{Security Evaluator}
\label{Section:Security Evaluator}
 This module will analyze the workflows in terms of security to check the potential security vulnerabilities in the workflow model. Also, this analysis will lead to creating propagation and separation patterns of the workflow that will be used in the next steps of workflow execution. The \textit{"separation patterns"} define some confidentiality requirements for each workflow to preserve data and logic privacy for different entities including instances, users, and tenants. These patterns are used in the scheduling phase to select the proper resources and services from suitable clouds. The \textit{"propagation patterns"} identify the effect of different violations in each task on the other tasks in a workflow. Based on these patterns, in the adaptation phase, we can discover which other tasks in a workflow should be adapted in addition to the violated task to prevent propagating the already occurred violations.
 In addition, the possible adaptation actions for each task are defined here. This requires establishing a set of adaptation strategies (e.g., skipping, re-working, re-sequencing) for each task in the workflow model and determining their potential impact on the overall value of the workflow and on the balance between value and security properties. As an example of such specification, consider the scenario of skipping certain tasks within the workflow, some tasks may be less critical, and skipping them may have little impact on the overall workflow value. However, for other tasks, such as authentication tasks, skipping is not even an option in case of any violation, as they are essential to the security of the workflow. In such cases, the impact of skipping could be significant and compromise the overall security of the workflow. Therefore, by incorporating such specifications for each task in the security evaluator module after the modeling phase, the cost of each adaptation action could be estimated in execution time, thus allowing to select the most viable adaptation option for any violations that may arise. 

==> Sections/draft_intro.tex <==

For example, applying the "insert" action when other tasks within the workflow have already been replaced due to prior violations may result in uncertain overhead costs. Similarly, applying the "skip" action to multiple specific tasks can introduce unhandled overhead, prolonging both the time and cost implications throughout the workflow.


Furthermore, the cloud is often considered honest but curious, meaning that the cloud service provider may faithfully follow the established protocols but, at the same time, maybe curious to deduce valuable information about the users' data and the workflow logic. This curiosity can potentially lead to the leakage or sale of deduced information to third parties by malicious cloud providers \cite{Liu2014}. Consequently, some users are reluctant to fully embrace cloud computing due to concerns about data privacy and security. 



can you specify a percentage effect for each of objctives in CIANA in probe,
DOS, u2r, r2l attacks. for example DOS thereat confidentilaity with this per-
centage It is difficult to provide specific percentages for the impact of different
cyberattacks on each of the CIANA security objectives because the impact can
vary widely depending on a number of factors, including the specific attack vec-
tor, the security measures in place, and the particular system being targeted.
However, I can provide a general overview of the potential impact of each attack
on each of the CIANA security objectives:
Probe Attacks:
Confidentiality: Probe attacks have the potential to breach confidentiality,
but the impact will depend on the specific information that is accessed. The
percentage effect cannot be estimated as it can vary widely. Integrity: Probe
attacks generally do not have a direct impact on data integrity. The percentage
effect is likely to be low or negligible. Availability: Probe attacks generally
do not have a direct impact on availability. The percentage effect is likely to
be low or negligible. Non-Repudiation: Probe attacks generally do not have a
direct impact on non-repudiation. The percentage effect is likely to be low or
negligible. Authenticity: Probe attacks generally do not have a direct impact
on authenticity. The percentage effect is likely to be low or negligible. Denial-
of-Service (DoS) Attacks:
Confidentiality: DoS attacks can lead to a breach of confidentiality if the
system is unavailable, and an attacker can gain unauthorized access during the
attack window. The percentage effect can vary widely depending on the specific
system being targeted and the nature of the information that may be exposed,
but it can be high in some cases. Integrity: DoS attacks generally do not
have a direct impact on data integrity. The percentage effect is likely to be
low or negligible. Availability: DoS attacks aim to disrupt the availability of
a system, making it unavailable to legitimate users, which can cause a breach
of availability. The percentage effect can be high, particularly if the system is
critical to business operations or public safety. Non-Repudiation: DoS attacks
generally do not have a direct impact on non-repudiation. The percentage effect
is likely to be low or negligible. Authenticity: DoS attacks generally do not
1
have a direct impact on authenticity. The percentage effect is likely to be low
or negligible. User-to-Root (U2R) Attacks:
Confidentiality: U2R attacks can result in the theft of sensitive data, which
can breach confidentiality. The percentage effect can vary widely depending
on the nature of the information that is stolen, but it can be high in some
cases. Integrity: U2R attacks can modify data, which can breach integrity.
The percentage effect can be high, particularly if the modified data is critical
to business operations or public safety. Availability: U2R attacks can crash a
system or make it unavailable, which can breach availability. The percentage
effect can be high, particularly if the system is critical to business operations
or public safety. Non-Repudiation: U2R attacks generally do not have a direct
impact on non-repudiation. The percentage effect is likely to be low or negli-
gible. Authenticity: U2R attacks can modify data and bypass authentication
mechanisms, which can breach authenticity. The percentage effect can be high,
particularly if the modified data is used for critical decisions. Remote-to-Local
(R2L) Attacks:
Confidentiality: R2L attacks can lead to the theft of sensitive data, which
can breach confidentiality. The percentage effect can vary widely depending
on the nature of the information that is stolen, but it can be high in some
cases. Integrity: R2L attacks can modify data, which can breach integrity. The
percentage effect can be
nafisesoezy@yahoo.com explain more about the impact can vary widely de-
pending on a number of factors, including the specific attack vector, the security
measures in place, and the particular system being targeted. The impact of a
cyberattack on the security objectives of a system can vary widely depending
on several factors. Here are some of the most important factors that can affect
the impact of a cyberattack:
Attack vector: The specific attack vector used by the attacker can have a
significant impact on the system’s security objectives. For example, some types
of attacks may be more effective at breaching confidentiality, while others may
be more effective at disrupting availability.
Security measures in place: The effectiveness of the security measures in
place can greatly affect the impact of a cyberattack. Systems that are well-
protected with strong security measures, such as firewalls, intrusion detection
and prevention systems, and data encryption, are less likely to be successfully
attacked than systems with weak or no security measures.
Particular system being targeted: The impact of a cyberattack can also vary
depending on the particular system being targeted. For example, an attack on a
system that contains sensitive financial data will likely have a greater impact on
confidentiality than an attack on a system that contains only public information.
Timeframe: The timeframe during which a cyberattack occurs can also affect
the impact of the attack. For example, an attack that occurs during a time of
high traffic or system usage may have a greater impact on availability than an
attack that occurs during a low traffic or low usage period.
Attackers’ motivation and skill level: The motivation and skill level of the
attacker can also have a significant impact on the success of a cyberattack. A
2
highly motivated and skilled attacker may be able to breach even the most well-
protected systems, while a less motivated or less skilled attacker may be easily
thwarted by basic security measures.
Given these factors, it is difficult to provide specific percentages for the im-
pact of different cyberattacks on each of the CIANA security objectives. It
is important for organizations to regularly assess their systems and security
measures and implement appropriate safeguards to mitigate the risks of cyber-
attacks.
nafisesoezy@yahoo.com can you specify a percentage effect for each of ob-
jctives in CIANA in R2L attack. It is difficult to provide specific percentages
for the impact of R2L (Remote-to-Local) attacks on each of the CIANA secu-
rity objectives, as the impact can vary depending on the specific attack vector,
security measures in place, and the particular system being targeted. However,
here are some potential impacts of R2L attacks on each of the CIANA security
objectives:
Confidentiality: R2L attacks can potentially breach confidentiality by al-
lowing an attacker to gain unauthorized access to sensitive data or information
on a system. The percentage impact on confidentiality would depend on the
sensitivity of the data accessed and the level of access obtained by the attacker.
Integrity: R2L attacks can potentially compromise the integrity of a system
by allowing an attacker to modify or manipulate data or files on a system. The
percentage impact on integrity would depend on the extent of the modifications
made by the attacker and the criticality of the affected data or files.
Availability: R2L attacks can potentially disrupt the availability of a system
by causing it to crash or become unresponsive. The percentage impact on
availability would depend on the severity of the attack and the length of time
the system is affected.
Non-repudiation: R2L attacks can potentially compromise non-repudiation
by allowing an attacker to impersonate a legitimate user or tamper with logs
or audit trails to hide their actions. The percentage impact on non-repudiation
would depend on the extent of the tampering and the level of detail in the logs
or audit trails.
Again, the percentage impact of R2L attacks on each of the CIANA security
objectives would depend on the specific circumstances of the attack and the
system being targeted. It is important for organizations to regularly assess their
systems for vulnerabilities and implement appropriate safeguards to mitigate the
risks of R2L attacks.



one of our novelty is our adversary model that consider different parties can be malicious.



In SaaS,the client has to depend on the provider for
proper security measures.The provider must do the workto
keep multiple users’from seeing each other’s data[1]
[1]A survey on security issues in service delivery models of cloud computing
S. Subashini n, V.Kavitha


https://www.orbussoftware.com/resources/blog/article/video-series-bpmn-pools-and-lanes#:~:text=A%20Pool%20represents%20a%20Participant,fully%20contained%20within%20the%20Pool.

for the lane and pool reduce the information disclure


WfMS is a field of management that can be defined as a paradigm that includes methods, techniques, and tools to support automated and seamless execution of workflows during whole workflow life cycle. It allows users to define and model workflows and then support workflows to enactment,management and analysis of operational processes. In general, it improves effectiveness and efficiency of the workflows in order to achieve lower costs, improve quality, and gain in productivity \cite{meidan2017survey,poola2017taxonomy}. 

workflow and life cycle

Cloud computing is a suitable platform for the execution of complex scientific and business processes that are described in the form of workflows. It can deliver a large amount of computing resources on demand for running data-intensive and compute-intensive applications. It also comes with the promise to reduce running costs and maximize revenues while maintaining or even improving the Quality of Service  \cite{survey}. Making use of cloud computing by Workflow Management Systems (WfMSs) can further increase the productivity of the system. In general, WfMSs are responsible for receiving the workflow input from the user and providing essential functionality to enable the execution of workflows such as task scheduling and service composition, managing the data-flow and control-flow dependencies, resource provisioning, and fault tolerance. \cite{Li2012a,Hwang2012,Rodriguez2017} 



Multi-tenancy is one of the important features of cloud-based WfMSs. In multi-tenant WfMS, each tenant can configure and run its workflow. The importance of this characteristic is that if each tenant deploys a separate WfMS independently of the other tenants, these multiple deployments will increase the burden of the workflow system, prolong the response time and reduce the execution efficiency \cite{Huang2019}. However, this feature can compromise the security and privacy of the running workflows that are belonging to different tenants. So, there is a need for a WfMS that provide an isolated execution and monitoring environment for each tenant. Such a system should be able to 1) distinguish the information of the workflow instance belonging to different tenants at run-time, 2) protect the confidentiality and integrity of the workflow' assets in the execution process of tenants’ workflow instances, 3) meet various functional and non-functional requirements of the different tenants \cite{Huang2019}. For this purpose, \cite{Huang2019} proposed a framework for the cloud workflow engine that can support privacy protection between mass various different tenant workflow instances in the cloud workflow systems. It provided this protection by using a separate tenant process virtual machines (namely the TPVM) created in the engine. However, in this paper, privacy is the only considered security factor. Besides, if one malicious tenant tries to compromise the other tenant's workflow instances, the system can not detect it. To put it better, it doesn't have any mechanisms in order to detect the security attacks occurred in the cloud or/and in the engine.

To the best of our knowledge, there is no WFMS that can support multi-tenancy considering security aspects during the whole workflow life cycle including Modeling, IT refinement, Deployment, Execution, Monitoring, Analysis, and Adaptation. Therefore, in this paper, we want to propose a multi-tenant WFMS that can handle all of the security concerns during all phases of the workflow life cycle in the multi-cloud environment. This multi-tenancy of the WfMS, in addition to the aforementioned benefits, can also help to detect the security and privacy violations with more precision as more data is collected from the different tenants. This data is about the violations of the different cloud services that happened in the running instances of various tenants. Besides, it can improve adaptation strategies in order to react and prevent. As an example, a detected security violation in one host can inform the other tenant's engines to prevent scheduling instances on that host or can alert the already running instance to migrate to another healthy host.


Both types of workflows (scientific and business) need to satisfy the fundamental security principles of CIANA (Confidentiality, Integrity, Availability, Non-Repudiation, and Authenticity) during the whole workflow life cycle. 

  The remainder of this paper is structured as follows. 




==> Sections/relatedWorkold.tex <==
\section{Related works}
In this section, we discuss existing monitoring and adaptation mechanisms for security violations in workflows outsourced to multi-cloud environments

 \begin{table*}[h!]
%\small
\fontsize{8pt}{10pt}\selectfont
\caption{{Different WfMSs regarding security concerns in the cloud.} }
\label{table1}
\def\arraystretch{1}
\ignorespaces 
%\centering 
\input{tables/table1}
\end{table*}

 \cite{HosseiniShirvani2020} addressed the web service composition problem in a multi-cloud environment by utilizing security logs to quantify Cloud Security Risk (CSR) and formulating it as a bi-objective optimization problem. They focused on minimizing service costs and mitigating multi-cloud risk through improved process design. However, the study did not incorporate dynamic trust calculation for providers based on occurred violations, limiting its adaptability to the dynamic cloud environment. 

In their paper, \cite{Wang2020b} proposed an intrusion tolerant scientific workflow system. They introduced a temporary workflow intermediate data backup strategy to preserve intermediate data for potential re-execution of sub-tasks with low confidence. The confidence of tasks is assessed through a lagged decision mechanism, providing assessments after task execution. Building on their previous work, \cite{Wang2021} addressed a limitation by scheduling replicas of sub-tasks to prevent the compromise of a single virtual machine from affecting the entire workflow. This adaptive technique adds redundancy to avoid executing compromised workflows from the beginning. However, the paper focuses solely on detecting integrity violations during the execution phase of scientific workflows and does not cover other types of security violations.

In \cite{Wen2020b}, the researchers proposed a dynamic rescheduling method to handle changes in cloud resource availability, such as failures or the availability of new resources. The cost model calculates the cost of deploying incomplete tasks on available resources and reschedules them to address runtime failures. This work focuses on resource availability as the main security factor and considers rescheduling as an adaptive action to address resource availability issues during the execution of scientific workflows.

The paper \cite{Abazari2019} introduces an attack response approach to mitigate security threats in scientific workflows. The approach involves calculating the security threat by assuming one task as malicious and estimating the number of affected tasks. If any malicious behavior is detected in a virtual machine (VM), the attack response module reschedules high-risk tasks, including both running and future tasks, as an adaptation strategy.

The paper \cite{Ahmad2021} presents a fault-tolerant workflow management system designed for scientific workflows in cloud computing. The system incorporates Quality-of-Service (QoS) aware scheduling to improve workflow execution. Its main aim is to efficiently allocate resources and handle faults that may occur during workflow execution. In case of job or task failures, the system employs a fault-tolerant approach to re-execute the failed tasks as its adaptation strategy. However, it primarily focuses on detecting violations leading to task failures rather than addressing other types of violations.

The paper \cite{Alaei2021b} presents an adaptive fault detector strategy for scheduling scientific workflows in the cloud. It integrates proactive and prescriptive adaptation techniques to handle faults, with a particular emphasis on VM unavailability. Proactive adaptation utilizes a prediction model to anticipate resource load changes and enhance failure prediction accuracy. Prescriptive adaptation employs a reactive fault tolerance approach, allocating new VMs when a processor fails during workflow execution. However, the paper does not address security concerns beyond VM faults.

We conducted a comparison of the papers in Table \ref{table1}. However, none of them fully address all potential attacks that could compromise the CIA (Confidentiality, Integrity, Availability) of outsourced workflow tasks in multi-cloud environments. Furthermore, the available adaptation actions are not sufficiently comprehensive to effectively mitigate the risks associated with various types of violations.




==> Sections/system_overview-draft.tex <==

In \textit{SecFlow}, the security-aware management of workflows can be divided into two main phases: the pre-submission phase (steps 1-4 in Figure \ref{fig:Architecture}), occurring before task submission to cloud environments, and the monitoring and adaptation phase (steps 5-11 in Figure \ref{fig:Architecture}), which detects and addresses security violations in cloud services and networks. In the following, we will discuss each of these steps in detail.

Based on our assumption that each tenant has a separate instance of the WfMS, the \textbf{Tenant's Kernel} provides an isolated environment for each tenant. The pre-submission phase of the workflow involves the following steps: 1) Tenants model their workflows based on security requirements (CIA) using the \textbf{\textit{Workflow Modeller}} module. 2) Workflows are analyzed using the \textbf{\textit{Security Evaluator}} module to define potential adaptation actions (e.g., skipping, re-working, re-sequencing, and re-configuration) for each task. 3) The \textbf{\textit{Security Evaluator}} module removes unnecessary sensitive information from the tasks before submission to the middleware. This module employs client-side obfuscation techniques such as data removal, noise injection, and data splitting, along with conflict detection methods to address conflicts between data minimization and security requirements \cite{Ramadan2020}. 4) The \textbf{\textit{Trust-aware Service Composition}} in the middleware schedules workflows and allocates cloud resources and services, considering tenant requirements and integrating trustworthiness information from the Provider Trust module. Task specifications are anonymized before execution in the cloud, similar to the Task Anonymizer module operating on the tenant side.

After submitting the workflow tasks to cloud resources and services for execution, the monitoring and adaptation procedure begins, involving the following steps: 5) The \textbf{\textit{Service Monitoring}} module continuously analyzes real-time network traffic data and cloud log files to detect any malicious activity in cloud services, providers, and the network. 6) It compares the monitored data with the expected behavior derived from the model trained by the \textbf{\textit{Service and Network Model Trainer}} module. If anomalies or suspicious activity are detected, the \textbf{\textit{Service Monitoring}} module raises an immediate alert to the corresponding tenant's adaptation module, prompting appropriate measures. 7) The \textbf{\textit{Adaptation Decision Engine}} selects the most suitable adaptation option for the identified attack, employing two distinct strategies. The first strategy prioritizes actions that impose minimal impact on the system, taking into consideration factors such as price, time, value, and mitigation score. 8) The second strategy involves utilizing an adaptive model, trained by the \textit{Adaptation Model Trainer} module, which takes into account system reactions, current workflow state, workflow dependencies, and potential execution uncertainties. 

After selecting the most appropriate adaptation action using one of these strategies, the necessary adaptations are implemented using different modules. These modules are categorized into two levels: tenant-level and middleware-level.


9) At the tenant level, the \textbf{\textit{Tenant Adapt Module}} is responsible for executing selected adaptation actions specific to individual tenants. These actions may involve task skipping, process re-sequencing (such as Late), or the introduction of new tasks (Insert). The purpose of this module is to mitigate any negative impact while preserving tenant privacy. 


 The middleware-level actions focus on managing adaptations related to changes in providers and cloud services. The middleware adaptation module plays a crucial role in handling these middle-level adaptations, relieving tenants from associated complexities and challenges. This approach allows tenants to concentrate on their tasks and responsibilities while the middleware adaptation module efficiently handles the necessary adjustments in the underlying infrastructure. Middleware-level actions primarily involve re-configuration and task re-execution. 10) The \textbf{\textit{Service Adaptation Module}} provides the capability to re-execute tasks when violations are detected. It implements necessary actions to meet evolving tenant requirements, including modifying selected services within the same provider or exploring alternatives from different providers. 11) Configuration adaptation focuses on adjusting the settings of specific cloud services to enhance decision-making. The middleware serves as a central point for receiving feedback from other tenants, establishing a trust factor for each provider and their services. Leveraging this collective information, the middleware can make informed decisions and execute adaptations that improve the reliability and performance of the system for all tenants. For this purpose, the \textbf{\textit{Provider Trust Module}} updates the trust score or level of the service and provider based on detected violations. The trust repository, containing information about providers and services, is updated accordingly. These updates enhance future scheduling decisions within the Trust-aware Service Composition module, enhancing overall security and efficiency. Additionally, this module may adjust the service and network model to improve the precision of monitoring malicious provider behavior.











\section{System Overview}
\label{sec:System Overview}
This section presents SecFlow, an innovative architecture specifically developed to efficiently handle and mitigate potential violations within multi-cloud environments during the execution of workflows. The main aim of our research is to proactively detect and address security threats posed by potential adversaries, focusing specifically on those originating from the cloud and network domains. In multi-tenant and cloud-based WfMS, various entities have the potential to compromise the sensitive resources of tenants which are outsourced to the cloud.



Moreover, we will provide a comprehensive overview of the entire detection and adaptation process employed by SecFlow to identify and adapt to violations occurring in cloud services and networks.

\subsection{Adversary Model}
In multi-tenant and cloud-based WfMS, various entities have the potential to compromise the sensitive resources of tenants which are outsourced to the cloud. This section discusses the details of these potential attackers. 

In a multi-tenant environment, \textbf{tenants} themselves have the potential to become threat actors. Malicious tenants can launch various attacks to compromise the assets of other tenants. Their objectives may involve unauthorized access to sensitive information, manipulation of tasks and data, or causing disruptions.

The cloud-based \textbf{WfMS} is responsible for providing essential functionality to manage the execution of the workflows which are submitted by tenants. While it is assumed to be semi-trusted and compliant with protocols, it may attempt to gather as much information as possible about tenants and their sensitive data.

\textbf{Cloud providers}, whose infrastructure and services are utilized by the WfMS for executing workflow tasks, can also be considered potential threat actors as semi-trusted parties. They have the ability to exploit tenants' assets, thus posing a significant security risk.

The shared nature of cloud infrastructure, where multiple users utilize computing and storage resources, introduces vulnerability to attacks. \textbf{External Attackers}, including malicious cloud provider users or individuals outside the cloud network (e.g., network attackers), exploit the Internet to execute disruptive attacks, thereby impacting the services available to legitimate users. In our specific case, these actors can target tenant assets during their execution within the cloud providers or even during data transfer processes.

\subsection{System Architecture}
\label{subSec:System Architecture}
This section presents an overview of our security-aware Workflow Management System (WfMS), called \textit{SecFlow}. It is specifically designed to provide comprehensive protection for workflows throughout their entire lifecycle, safeguarding them against a wide range of security violations and ensuring defense against all potential attackers. Figure \ref{fig:Architecture} provides a detailed illustration of the proposed architecture, highlighting key components such as the Tenant's Kernel, the Middleware, and the multi-cloud environment.

In our architecture, we assume that tenants' resources are securely isolated from each other, possibly residing on the same cloud node. The middleware, which acts as a logically centralized component, can be hosted by a trusted third party. In this architecture, tenants actively participate in monitoring their users, while the Middleware component supervises the behavior of both the Clouds and the tenants, leveraging behavioral patterns learned from both sides. Since our focus in this paper is on detecting security violations in the cloud service and network, we describe the detection and adaptation procedures using the \textit{SecFlow} architecture in the following. 

\begin{figure*}[h]
  \includegraphics[width=\textwidth]{figures/system model-paperDetect.pdf}
  \caption{The architecture of SecFlow}
  \label{fig:Architecture}
\end{figure*}

In \textit{SecFlow}, the security-aware workflow management consists of two phases: the pre-submission phase, which occurs before task submission to cloud environments, and the monitoring and adaptation phase, which detects and addresses security violations in cloud services and networks.

Based on our assumption that each tenant has a separate instance of the WfMS, the \textbf{Tenant's Kernel} provides an isolated environment for each tenant. The pre-submission phase of the workflow involves the following steps: 1) Tenants model their workflows based on security requirements (CIA) using the \textbf{\textit{Workflow Modeller}} module. 2) Workflows are analyzed using the \textbf{\textit{Security Evaluator}} module to define potential adaptation actions (e.g., skipping, re-working, re-sequencing, and re-configuration) for each task. 3) The \textbf{\textit{Security Evaluator}} module removes unnecessary sensitive information from the tasks before submission to the middleware. This module employs client-side obfuscation techniques such as data removal, noise injection, and data splitting, along with conflict detection methods to address conflicts between data minimization and security requirements \cite{Ramadan2020}. 4) The \textbf{\textit{Trust-aware Service Composition}} in the middleware schedules workflows and allocates cloud resources and services, considering tenant requirements and integrating trustworthiness information from the Provider Trust module. Task specifications are anonymized before execution in the cloud, similar to the Task Anonymizer module operating on the tenant side.

After submitting the workflow tasks to cloud resources and services for execution, the monitoring and adaptation procedure begins, involving the following steps: 5) The \textbf{\textit{Service Monitoring}} module continuously analyzes real-time network traffic data and cloud log files to detect any malicious activity in cloud services, providers, and the network. 6) It compares the monitored data with the expected behavior derived from the model trained by the \textbf{\textit{Service Model Trainer}} module. If anomalies or suspicious activity are detected, the \textbf{\textit{Service Monitoring}} module raises an immediate alert to the corresponding tenant's adaptation module, prompting appropriate measures. 7) The \textbf{\textit{Adaptation Decision Engine}} selects the most suitable adaptation option for the identified attack, employing two distinct strategies. The first strategy prioritizes actions that impose minimal impact on the system, taking into consideration factors such as cost, time, mitigation effectiveness. The second strategy involves utilizing a predictive model to predict the best adaptation action for the detected attack  8) This predictive model used in strategy two is trained by the \textit{Adaptation Model Trainer} module based on the system reactions considering the current state of the workflow and the workflow dependencies and also the uncertainty that may occur during the execution. 9) The \textbf{\textit{Tenant Adapt Module}} performs selected adaptation actions at the tenant level, such as skipping tasks, re-sequencing processes, or introducing new tasks to mitigate the impact. 10) The \textbf{\textit{Service Adaptation Module}} handles selected adaptation actions at the middleware level, enabling the adaptation of services chosen by the Adaptation Decision Engine. It implements necessary actions to meet evolving tenant requirements, including modifying selected services within the same provider or exploring alternatives from different providers. 11) Based on the detected violation, the \textbf{\textit{Provider Trust Module}} updates the trust score/level of the service and provider. The trust repository of providers and services is updated, improving scheduling decisions for future workflow instances. The Trust-aware Service Composition utilizes updated trust values to schedule upcoming workflow instances, enhancing overall security and efficiency. Additionally, this module may modify the Provider Prediction model to improve the monitoring of malicious provider behavior with greater precision.

It is important to note that due to the extensive scope of the architecture, this paper does not delve into certain modules, namely the \textit{Tenant's Rule-based Intrusion Detection System (IDS)} for detecting tenant-originated attacks, the \textit{Tenant Trust Module} for adapting malicious behavior from tenants, and the \textit{Tenant's Detection module (Local Detection)} for detecting and monitoring malicious user behavior using a pre-trained model. The inclusion of these modules in this paper is intended to provide a comprehensive overview of the entire architecture. However, further work and discussion will be dedicated to these modules in future research.

\subsection{Privacy Preservation and Efficient Adaptation Handling}
By differentiating between tenant-level and middleware-level actions, we serve multiple purposes, including the preservation of tenant privacy and the efficient handling of middle-level adaptations. Tenant-level actions are specifically designed to safeguard tenant privacy by implementing strategies and adaptations tailored to their specific requirements. These actions leverage the tenant's own strategies and the task-level adaptation module to ensure the security of sensitive information and maintain privacy during the adaptation process. Tenant actions involve tasks skipping and re-sequencing, and it is the responsibility of the tenant to apply these adaptation actions according to their preferences.

On the other hand, middleware-level actions focus on managing adaptations associated with changes in providers and cloud services. The middleware adaptation module plays a crucial role in relieving tenants from the complexities and challenges of middle-level adaptations. This approach allows tenants to concentrate on their tasks and responsibilities while the middleware adaptation module efficiently handles the necessary adjustments in the underlying infrastructure. Additionally, the middleware serves as a central point for receiving feedback from other tenants, establishing a trust factor for each provider and their services. Leveraging this collective information, the middleware can make informed decisions and execute adaptations that enhance the reliability and performance of the system for all tenants.

Middleware-level actions primarily involve re-configuration and task re-execution in the adaptation process. Configuration adaptation focuses on adjusting the settings of specific cloud services to improve decision-making in various modules. This includes modifying the trust level of cloud services within the Service Composition
 module and adjusting the Attack Frequency Rate (AFR) used in the Adaptation Decision Engine to calculate the attack score. Alongside configuration adaptation, the middleware adaptation module offers the option of re-executing tasks in case of detected violations. This allows the navigator to respond to security breaches by re-running affected tasks with modifications or alternative approaches to ensure workflow security. There are two options available for task re-execution. The first option is to continue running the task with the same cloud provider while implementing additional security measures. This involves utilizing a different Service Level Agreement (SLA) that provides enhanced security guarantees. The navigator can negotiate with the cloud provider to enforce stricter security controls, particularly for data transfer. This option is suitable when the violation is detected in network traffic data, indicating no malicious behavior within the cloud services. The second option is to re-run the task using a different cloud provider. In this scenario, the navigator switches to a different cloud provider to achieve a higher level of security and reduce the likelihood of future security violations. This option is chosen when the violation is detected in the cloud log file, indicating malicious cloud behavior or an ongoing attack.

 



==> table1.tex <==
\begin{table*}[ht]
\caption{Possible Attacks in the Workflows}
\centering
\begin{tabular}{p{0.187\linewidth}|p{0.187\linewidth}|p{0.187\linewidth}|p{0.187\linewidth}}
\hline
Type of Attack & Related Attacks & Potential Targets in Workflow  & Implications of attacks \\
\hline
Application-based Attack & Fault injection, Inference Attack,
Account Hijacking, web service and protocol based attacks

& Fragment(group of tasks)
Data(Input/Output)
Message(Send/Receive)
Task(Code/Service), Control Flow Connector & Malicious manipulation of data,
Violation of data protection,
Denial-of-service\\

\hline

Network-based Attack &   port scanning, botnets, spoofing attacks, eavesdropping attack,the man-in-the-middle attack, and the replay attack     & Data(Input/Output)
Message(Send/Receive)
 Task(code/Service) &
Violation of data protection,
Denial-of-service
 \\
\hline


VM-based Attack & Cross VM   side channel attacks
VM creation attacks
VM migration and roll back attacks
VM scheduler based attacks(VM escape, VM hopping, etc.) &
Data(Input/Output)
Message(Send/Receive)
 Task(code/Service) & Violation of data protection
Denial-of-service  \\
\hline
\end{tabular}
\end{table*}


==> tables/table1_back.tex <==
\begin{tabulary}{\linewidth}{ p{3cm}p{1.7cm}p{1.7cm}p{1.7cm}p{1.8cm}p{1.7cm}p{1.7cm}}

 \textbf{Paper} &
\textbf{Type of Workflow}  & 
\textbf{Monitoring Module}  &
\textbf{Considered Security Objectives} &
%\textbf{Considered Attacker} &
\textbf{Considered Attack} &
\textbf{Adaptation Options}  
\\  \hline  \hline

%\cite{HosseiniShirvani2020}, 2020 &	Business workflows & Cloud-side Monitoring & CIA & -	& anomalies such as virtualisation and network attacks and security breaches & Reconfiguration(change trust) based on the cloud logfile
 %\\\hline

% \cite{Rekik2016}, 2016 &	Business workflows & Engine-side Monitoring & - & -	& -& -
 %\\\hline

 \cite{Wang2020b}, 2020
\cite{Wang2021}, 2021 &	Scientific workflows	& Engine-side Monitoring & I & External Attacker & VM-based attacks & Redundancy
 \\\hline

  \cite{Wen2020b}, 2020	& Scientific workflows	& Cloud-side Monitoring & A & attacks that can change the resource availability	& Clouds fail and Availability
of new clouds. & Rescheduling the uncompleted services
 \\\hline
 
 \cite{Abazari2019}, 2018	& Scientific workflows & The Cloud Administrator module & CIA & Cloud insider, External attacker	& VM-based attacks & Rescheduling the affected tasks
 \\\hline
 
 \cite{Ahmad2021},2021 &	Scientific workflows & Engine-side Monitoring & A & -	& hardware/software faults & Re-work
 \\\hline
 
 \cite{Alaei2021b}, 2021 &	Scientific workflows & Engine-side Monitoring & A & attacks that can change the resource availability & unavailability of VMs	& Re-work
 \\\hline


\end{tabulary}\par 

==> tables/table2.tex <==
\begin{table}[ht]
\caption{Parameters and Definitions}
\label{table:parameters}
\begin{tabular}{ll}
\hline
\textbf{Parameter} & \textbf{Definition} \\
\hline
$a_k$: Detected Attack, $t_i$: Current Task, $s_j$: Current Service, $l_{a_k}$: Attack Severity Level, $Tenant.attackThresh$: Attack Threshold, $AA_{l_{a_k}}$: Adaptation Actions for Mitigation, $AA_{t_i}$: Feasible Adaptation Actions for Current Task




APM & Attack Prediction Model \\
CLF & Cloud Log File \\
NTD & Network Traffic Data \\
AttackType & A \\
 $a_k$ & Detected Attack \\
  $l_{a_k}$ & Attack's severity level of detected attack learned by the algorithm \ref{alg:attack_severity_learning}\\
  $t_i$ &  Current Task \\
 $s_j$ & Current Service  \\
 $(AT_{a_k})$ & Attacktype of detected attack\\
$AFR_{s_j}(A_{a_k})$ & AFR of the current service for the Attacktype of detected attack.
$Tenant.attackThresh$ & Attack Threshold of the current tenant \\
$AA$ & Total potential adaptation actions for the detected attack in a specific task \\
$aa$ & The Adaptation Action \\
$Selectedaa$ & The Selected Adaptation Action
AttackTypes & List of AttackTypes\\

 $a_k$: Detected Attack, $t_i$: Current Task that attack is detected, $s_j$: Current Service that attack happen on it, $l_{a_k}$: Attack's severity level for detected attack, $Tenant.attackThresh$: Attack Threshold of the current tenant that own workflow, $AA_{l_{(a_k_)}}$: the adaptation actions that can be taken to mitigate the impact of the detected attack, $AA_{t_i}$:  the feasible adaptation actions that can be performed on the current task

\hline
\end{tabular}
\end{table}

\begin{table}[ht]
\caption{Parameters and Definitions}
\label{table:parameters}
\begin{tabular}{llll}
\hline
\textbf{Parameter} & \textbf{Definition} & \textbf{Parameter} & \textbf{Definition} \\
\hline
APM & Attack Prediction Model & $a_k$ & Detected Attack \\
CLF & Cloud Log File & $l$ & Attack's severity level of detected attack \\
NTD & Network Traffic Data & $t_i$ & Current Task \\
AttackType & A & & Current Service $s_j$ \\
 & & Tenant.attackThresh & Attack Threshold of the current tenant \\
AA & Total potential adaptation actions for the detected attack in a specific task & aa & The selected adaptation action \\
\hline
\end{tabular}
\end{table}

==> tables/table3.tex <==
\newcolumntype{L}[1]{>{\raggedright\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}

\begin{tabulary}{\linewidth}{ L{1.8cm}L{1.5cm}L{1.9cm}L{1.5cm}L{1.9cm}L{1.9cm}L{1.5cm}}

 
 \textbf{Adaptation Actions} &
\textbf{Incident Details}  & 
\textbf{Hospital Report}  &
\textbf{Police Report} &
\textbf{Expert Report}&
\textbf{Bank Reimbursement}  &
\textbf{Customer feedback collection} 
\\  \hline  \hline

\textbf{Late} &
$R/2$,$P$,$V/2$  & $R/2$,$P$,$V/3$  & $R/2$,$P$,$V/3$  & \multicolumn{1}{c}{-}  & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-}
\\  \hline

\textbf{Insert} &
\multicolumn{1}{c}{-}  & $R*2$,$P$,$V$  & $R/2$,$P*3$,$V$  & $R/2$,$P*2$,$V/2$  & $R/2$,$P*2$,$V/5$ & $R*2$,$P*3$,$V$
\\  \hline

\textbf{Skip} &
\multicolumn{1}{c}{-}  & \multicolumn{1}{c}{-}  & \multicolumn{1}{c}{$0$, $0$, $0$}  & \multicolumn{1}{c}{-}  & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{$0$, $0$, $0$}
\\  \hline


\textbf{Rework} &
\multicolumn{6}{c}{$R_{BackupSrc}$ , $P_{BackupSrc}$ , $V$}
\\  \hline

\textbf{Redundancy} &
\multicolumn{6}{c}{$R_{BackupSrc}$ , $P+P_{BackupSrc}$ , $V*2$}
\\  \hline


\textbf{Reconfig} &
\multicolumn{6}{c}{$R*T_{reconfig}$ ,  $P*P_{reconfig}$ ,  $R*V_{reconfig}$}
\\  \hline

\bottomrule 
\end{tabulary}\par 



==> tables/table5.tex <==
\newcolumntype{L}[1]{>{\raggedright\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}

\begin{tabulary}{\linewidth}{ L{7cm}L{2cm}}

   
\textbf{Information}  & 
\textbf{Range}  
\\  \hline


Average Response Time &
[1 ... 50]
\\  \hline

Cost  &
[0.1 ... 10]
\\  \hline

Confidentiality  &
[0 ... 1]
\\  \hline

Integrity  &
[0 ... 1]
\\  \hline

Availability &
[0 ... 1]
\\  \hline
 
\bottomrule 
\end{tabulary}\par 
